Deep Learning-Based Out-of-distribution Source Code Data Identification: How Far Have We Gone?

Software vulnerabilities (SVs) have become a common, serious, and crucial concern to safety-critical security systems. That leads to significant progress in the use of AI-based methods for software vulnerability detection (SVD). In practice, although AI-based methods have been achieving promising performances in SVD and other domain applications (e.g., computer vision), they are well-known to fail in detecting the ground-truth label of input data (referred to as out-of-distribution, OOD, data) lying far away from the training data distribution (i.e., in-distribution, ID). This drawback leads to serious issues where the models fail to indicate when they are likely mistaken. To address this problem, OOD detectors (i.e., determining whether an input is ID or OOD) have been applied before feeding the input data to the downstream AI-based modules. While OOD detection has been widely designed for computer vision and medical diagnosis applications, automated AI-based techniques for OOD source code data detection have not yet been well-studied and explored. To this end, in this paper, we propose an innovative deep learning-based approach addressing the OOD source code data identification problem. Our method is derived from an information-theoretic perspective with the use of innovative cluster-contrastive learning to effectively learn and leverage source code characteristics, enhancing data representation learning for solving the problem. The rigorous and comprehensive experiments on real-world source code datasets show the effectiveness and advancement of our approach compared to state-of-the-art baselines by a wide margin. In short, on average, our method achieves a significantly higher performance from around 15.27%, 7.39%, and 4.93% on the FPR, AUROC, and AUPR measures, respectively, in comparison with the baselines.

==> sections/discussion.tex <==
\subsection{\textbf{Threats to validity }}

\paragraph{\textbf{Construct validity}}
Key construct validity threats are if the assessments of our proposed \ourapp~method and baselines demonstrate their capability for out-of-distribution source code data identification. In the cyber security domain, the out-of-distribution source code data identification task helps determine if an input is from an in-distribution (ID) or out-of-distribution (OOD). That enables the model and security experts to take appropriate precautions and actions. In particular, this stage assists security analysts and software engineers in identifying potential out-of-distribution CWE source code data outside the established in-distribution CWE source code data categories before feeding input data into subsequent machine learning and deep learning modules, to harden the software security systems. To evaluate the performance of our \ourapp~method and baselines, we use three main measures widely used in out-of-distribution detection including FPR (at TPR 95\%), AUROC, and AUPR.

\paragraph{\textbf{Internal validity}}
Key internal validity threats are relevant to the choice of hyper-parameter settings (i.e., optimizer, learning rate, number of layers in deep neural networks, etc.). It is worth noting that finding a set of optimal hyperparameter settings of deep neural networks is expensive due to a large number of trainable parameters. To train our method, we only use the common or default values for the hyperparameters. For example, we use the Adam optimizer; the learning rate equals $10^{-3}$; the size of neural layers is set in $\{100, 300\}$ while the scalar temperature $\tau$ used in the cluster-contrastive learning and the temperature $\nu$ for the Gumbel softmax distribution is set in $\{0.5, 1.0\}$. For the number of clusters used in cluster-contrastive learning aiming to improve the data representation learning process, we use it as a hyperparameter. In our paper, we detail the hyperparameter settings (i.e., the value-tuned ranges of the hyperparameters) in the released reproducible source code to support future replication studies.

\paragraph{\textbf{External validity}}
Key external validity threats include whether our \ourapp~method will generalize across multiple CWE source code categories. We mitigated this problem by conducting the experiments on an up-to-date and big C/C++ dataset, \textit{namely DiverseVul}, \cite{chen2023diversevul}. The DiverseVul dataset contains 18,945 vulnerable functions and 330,492 non-vulnerable functions covering 150 CWEs. In our paper, we conduct the experiments on the top most dangerous and popular CWE categories including CWE-119 (Improper Restriction of Operations within the Bounds of a Memory Buffer), CWE-20 (Improper Input Validation), CWE-125 (Out-of-bounds Read), CWE-200 (Exposure of Sensitive Information to an Unauthorized Actor), CWE-787 (Out-of-bounds Write), CWE-416 (Use After Free), CWE-269 (Improper Privilege Management), CWE-94 (Improper Control of Generation of Code), CWE-190 (Integer Overflow or Wraparound), CWE-264 (Permissions, Privileges, and Access Controls), CWE-863 (Incorrect Authorization), CWE-862 (Missing Authorization), and CWE-287 (Improper Authentication).



==> sections/related_background.tex <==
\subsection{Related backgrounds}

In this section, we briefly present the main related backgrounds used in our proposed \ourapp~ and the baseline methods.

\subsubsection{\textbf{Recurrent neural networks}}

Recurrent neural networks (RNNs) \cite{Rumelhart-RNN86}, a class of deep neural networks (DNNs), are specialized for sequential data (e.g., time series, sentences, documents, or audio samples). RNNs are extremely useful for natural language processing (NLP) systems \cite{ChoMBB14,sutskever2014sequence}
such as automatic translation, speech-to-text, and sentiment analysis. Leveraging the idea of sharing parameters across different parts of a model, an RNN can extend and apply to data of different forms and generalize across them. An RNN is similar to a DNN, except it has backward connections.
A visualization of an RNN's architecture is depicted in Figure \ref{fig:architecture-of-rnn}
(the left-hand figure). At each time step $t$, the state of a recurrent
neuron (i.e., the hidden state denoted by $\bh_{t}$) will receive the input vector $\bx_{t}$ as well as the state vector from the previous step $t-1$ (i.e., $\bh_{t-1}$) to obtain the state vector $\bh_{t}$.

In particular, we have:
\[
\bh_{t}=f(\bh_{t-1},\bx_{t})
\]

We can unroll the RNN network through time to gain a new visualization as depicted in Figure \ref{fig:architecture-of-rnn} (the right-hand figure). Each recurrent neuron has two relevant input weights. One is for the input vector $\bx_{t}$, and the other is for the state vector $\bh_{t-1}$ of the previous time step $t-1$. At the time step $t$, if we denote the weight from the input vector $\bx_{t}$ to the state $\bh_{t}$ of the current recurrent neuron by $\bW_{xh}$ and the weight from the state $\bh_{t-1}$ of the previous recurrent neuron to the state $\bh_{t}$ of the current recurrent neuron by $\bW_{hh}$, the state $\bh_{t}$ of the current recurrent neuron is computed as follows:
\[
\bh_{t}=\phi(\bW_{xh}^{\top}\bx_{t}+\bW_{hh}^{\top}\bh_{t-1}+\bb)
\]

where $\bb$ is the bias vector and $\phi(.)$ is the activation function (e.g., the ReLU or Tanh functions).

At the time step $t$, if we denote $\bW_{hy}$ as the weight from the state $\bh_{t}$ of the current recurrent neuron to the corresponding output denoted by $\by_{t}$, the output $\by_{t}$ is computed as follows:

\[
\by_{t}=\phi(\bW_{hy}^{\top}\bh_{t}+\bc)
\]

where $\bc$ is the bias vector and $\phi(.)$ is the activation function (e.g., the softmax function).

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.96\columnwidth]{figures/RNN.png}
\par\end{centering}
\caption{An Architecture of a recurrent neural network with the outputs $y$ plus the hidden states $h$ of recurrent neurons. \label{fig:architecture-of-rnn}}
\end{figure}

\subsubsection{\textbf{Long short-term memory networks}}

Long short-term memory (LSTM) networks are a type of RNNs capable of learning long-term dependencies, first proposed by Hochreiter and
Schmidhuber \cite{hochreiter1997long-short} and gradually improved over the years by other researches \cite{hasim-lstm-2014,zaremba-lstm-2014}. An LSTM network was introduced to address the exploding and vanishing gradients problems as well as the short-term memory problem (i.e., the lost information from some of the first elements from the corresponding input in the memory cell of a long RNN) in training RNNs.

The key idea of an LSTM network is about storing long-term memory. An LSTM network can learn to figure out what information from the inputs should be read and stored in the long-term state denoted by
$\bc_{t}$ as well as what information should be thrown out from $\bc_{t}$. A visualization of an LSTM network is shown in Figure \ref{fig:architecture-of-lstm}.
As depicted, there are four layers in an LSTM network including the main layer and three additional layers (i.e., gate controllers), namely, the forget gate, the input gate, and the output gate.
\begin{itemize}
\item The main layer at the time step $t$ aims to analyse the current input vector $\bx_{t}$ and the previous (short-term) state $\bh_{t-1}$ to gain the output $\bg_{t}$ (i.e., $\bh_{t}$ in a basic cell RNN). In an LSTM cell, the layer's output $\bg_{t}$ does not go straight out, but instead goes through a gate controller to decide what parts are stored in the long-term state (i.e., $\bc_{t}$).
\item Using the logistic activation function, the forget gate $\bff_{t}$ aims to learn which parts of the long-term state $\bc_{t}$ should be erased. The input gate $\bi_{t}$ aims to control which parts of $\bg_{t}$ should be added to the long-term state $\bc_{t}$ while the output gate $\bo_{t}$ aims to learn which parts of the long-term state $\bc_{t}$ should be outputted for both $\bh_{t}$ and $\by_{t}$.
\end{itemize}

The following equation (i.e., Eq. (\ref{eq:lstm})) summarises the computing process of the four layers of an LSTM network at the time step
$t$:
\begin{align}
\bi_{t} & =\sigma\left(\bW_{xi}^{\top}\bx_{t}+\bW_{hi}^{\top}\bh_{t-1}+\bb_{i}\right)\nonumber \\
\bff_{t} & =\sigma\left(\bW_{xf}^{\top}\bx_{t}+\bW_{hf}^{\top}\bh_{t-1}+\bb_{f}\right)\nonumber \\
\bo_{t} & =\sigma\left(\bW_{xo}^{\top}\bx_{t}+\bW_{ho}^{\top}\bh_{t-1}+\bb_{o}\right)\nonumber \\
\bg_{t} & =\tanh\left(\bW_{xg}^{\top}\bx_{t}+\bW_{hg}^{\top}\bh_{t-1}+\bb_{g}\right)\nonumber \\
\bc_{t} & =\bff_{t}\otimes\bc_{t-1}+\bi_{t}\otimes\bg_{t}\nonumber \\
\by_{t} & =\bh_{t}=\bo_{t}\otimes\tanh(\bc_{t-1})\label{eq:lstm}
\end{align}

where $\bW_{xi}$, $\bW_{xf}$, $\bW_{xo}$ and $\bW_{xg}$ are the weight matrices from the input vector $\bx_{t}$ to each of the four layers while $\bW_{hi}$, $\bW_{hf}$, $\bW_{ho}$ and $\bW_{hg}$ are the weight matrices from the previous short-term state $\bh_{t-1}$ to each of the four layers, and $\bb_{i}$, $\bb_{f}$, $\bb_{o}$ and $\bb_{g}$ are the bias vectors to each of the four layers, respectively.
In general, the output $\by_{t}$ can be different from the short-term state $\bh_{t}$ (i.e., $\by_{t}=\phi(\bW_{hy}^{\top}\bh_{t}+\bb_{y})$)
where $\bb_{y}$ is the bias vector while $\bW_{hy}$ is the weight from $\bh_{t}$ to $\by_{t}$, and $\phi(.)$ is the activation function (e.g., the softmax function).

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.95\columnwidth]{figures/LSTM.png}
\par\end{centering}
\caption{An architecture of a long short-term memory (LSTM) network. \label{fig:architecture-of-lstm}}
\end{figure}

\subsubsection{\textbf{Convolutional neural networks}}

Convolutional neural networks (CNNs) \cite{Lecun98gradient-basedlearning} are a kind of DNNs that are specialized for processing image data. CNNs have achieved breakthrough performance on many complex visual tasks \cite{alex_2012, TranBFTP15} such as visual object recognition, self-driving cars, automatic video classification systems, and more.
CNNs also successfully show high performance on other tasks such as voice recognition and natural language processing (NLP). In 1998, Lecun et al. \cite{Lecun98gradient-basedlearning}
introduced a typical famous architecture of a CNN named LeNet-5 as depicted in Figure \ref{fig:architecture-of-cnn}. This architecture shows some common building blocks often used in CNNs including fully
connected layers (i.e., as used in DNNs), convolutional layers, and pooling layers.

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.96\columnwidth]{figures/CNN.png}
\par\end{centering}
\caption{An architecture of LeNet-5 (a convolutional neural network) with some building blocks including convolutional layers, pooling layers, and fully connected layers. \label{fig:architecture-of-cnn}}
\end{figure}

\textbf{Convolutional layers} as shown in Figure \ref{fig:architecture-of-cnn} are the most important part of a CNN. The neurons in the first convolutional layer are connected to pixels in small rectangles (i.e., the receptive fields) of the input layer. This principle is kept for the connection between other layers (e.g., the connection between the second convolutional layer and the first convolutional layer). The neurons in the second convolutional layer are also connected to only some neurons in the first convolutional layer in the receptive fields. This architecture allows the network to concentrate on small low-level (i.e., general) features in some first hidden layers, and then assemble them into larger higher-level (i.e., specific) features in some next hidden layers. In reality, a convolutional layer often applies multiple \textbf{filters} (i.e., trainable filters and each filter outputting one feature map) to gain multiple corresponding \textbf{feature maps}, making the convolutional layer capable of detecting multiple features from its inputs.

We can summarise the computational process of convolutional layers by using Eq. (\ref{eq:cnn}) to further demonstrate how to compute the output of a given neuron
of a convolutional layer.

\begin{equation}
o_{i,j,k}=b_{k}+\sum_{u=0}^{f_{h}-1}\sum_{v=0}^{f_{w}-1}\sum_{k'=0}^{f_{k'}-1}o'_{i\times s_{h}+u,j\times s_{w}+v,k'}\times w_{u,v,k',k}\label{eq:cnn}
\end{equation}

where 
\begin{itemize}
\item $o_{i,j,k}$ is the output in row $i$ and column $j$ in the feature map $k$ of convolutional layer $l$.
\item $o'_{i\times s_{h}+u,j\times s_{w}+v,k'}$ is the output in row $i\times s_{h}+u$
and column $j\times s_{w}+v$ in the feature map $k'$ of the previous
convolutional layer $l-1$.
\item $w_{u,v,k',k}$ is the connection weight (i.e., it is updated during the training process) between any neuron in the feature map $k$ of convolutional layer $l$ and its inputs in row $u$ and column $v$ of the corresponding receptive field and feature map $k'$ of the
previous convolutional layer $l-1$ while $b_{k}$ is the bias of
the feature map $k$ of convolutional layer $l$.
\end{itemize}

The next important blocks of a CNN are pooling layers. The main goal of the \textbf{pooling layers} is to subsample (i.e., shrink) the input convolutional layer in order to reduce the computational cost. Pooling layers not only reduce memory usage but also reduce the number of parameters, thus eliminating the risk of overfitting. Pooling layers have no weights and they only aim to aggregate the inputs using an aggregation function such as the max or mean. We also need to define the size, the stride, and the padding type (i.e., zero padding or no padding) for the pooling layers.

It is worth noting that convolutional neural networks (CNNs) \cite{Lecun98gradient-basedlearning} were introduced and specialized for processing image data; However, they have also shown excellent performance when working on sequential data (e.g., text used in sentiment analysis \cite{Kim14f, ZhangW15b}).

\subsubsection{Transformers}

Transformer models \cite{transformers-Vaswani17, chatgpt} represent groundbreaking advancements in natural language processing and machine learning. These models have revolutionized various fields by demonstrating remarkable abilities in understanding and generating human-like text. Operating on a \textbf{self-attention mechanism}, transformers are uniquely adept at capturing contextual relationships in language, making them exceptionally proficient in natural language processing tasks such as language translation and text generation.

The architecture of a Transformer's framework is depicted in Figure \ref{fig:architecture-of-transformer}. In general, a Transformer follows the encoder-decoder structure used in neural sequence transduction models \cite{SutskeverVL14, Bahdanau15}. The encoder aims to map an input sequence of token representations $X=(\mathbf{x}_1,...,\mathbf{x}_n)$ to a sequence of continuous representations $Z=(\mathbf{z}_1,...,\mathbf{z}_n)$. Given $Z$, the decoder then generates an output sequence $Y=(\mathbf{y}_1,...,\mathbf{y}_n)$ of symbols one element at a time. At each step the model is auto-regressive \cite{Graves13}, consuming the previously generated tokens as additional input when generating the next token.

The encoder and decoder of a Transformer consist of multiple layers including multi-head attention layers and feed-forward neural networks. The main part of multi-head attention layers is the scaled dot product attention which is the core concept behind self-attention. In self-attention, each sequence element provides a key, value, and query. For each element, we perform an attention layer where based on its query, we check the similarity of all sequence elements’ keys and return a different, averaged value vector for each element.

\paragraph{\textbf{Scaled dot product attention}}

The core concept behind self-attention is the scaled dot product attention whose goal is to have an attention mechanism with which any element in a sequence can attend to any other while still being efficient to compute.

The dot product attention takes as input a set of queries $Q\in R^{L\times d_{k}}$, keys $K\in R^{L\times d_{k}}$, and values $V\in R^{L\times d_{v}}$ where $L$ is the sequence length and $d_{k}$ and $d_{v}$ are the hidden dimensionality for queries, keys, and values, respectively. The attention value from element $i$ to $j$ is based on its similarity of the query $Q_i$ and key $K_j$, using the dot product as the similarity metric. In math, we calculate the dot product attention as follows:

\[
Attention(Q,K,V)=softmax(\frac{QK^{T}}{\sqrt{d_{k}}})V
\]

where ${1}/{\sqrt{d_k}}$ is the scaling factor. The matrix multiplication $QK^{T}$ performs the dot product for every possible pair of queries and keys, resulting in a matrix of the shape $L\times L$. Each row represents the attention logits for a specific element to all other elements in the sequence. On these, we apply a softmax and multiply with the value vector to obtain a weighted mean (the weights being determined by the attention).

\paragraph{\textbf{Multi-Head Attention}}

The scaled dot product attention allows a network to attend over a sequence. However, often there are multiple different aspects a sequence element wants to attend to, and a single weighted average is not a good option for it. This is why the authors extend the attention mechanisms to multiple heads, i.e. multiple different query-key-value triplets on the same features. Specifically, given a query, key, and value matrix, we transform those into sub-queries, sub-keys, and sub-values, which we pass through the scaled dot product attention independently. Afterward, we concatenate the heads and combine them with a final weight matrix. Mathematically, we can express this operation as:

\begin{align*}
Multihead(Q,K,V) & =Concat(head_{1},...,head_{d})W^{O}\\
where\,\,head_{i} & =Attention(QW_{i}^{Q},KW_{i}^{K},VW_{i}^{V})
\end{align*}

In this multi-head attention computational process, $W_{1...h}^{Q}\in R^{D\times d_{k}}$, $W_{1...h}^{K}\in R^{D\times d_{k}}$,
$W_{1...h}^{V}\in R^{D\times d_{v}}$, and $W_{1...h}^{O}\in R^{h.d_{v}\times d_{out}}$ ($D$ being the input dimensionality) are the learnable parameters.

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{figures/Transformer.pdf}
\par\end{centering}
\caption{An architecture of the Transformer model \cite{transformers-Vaswani17}. \label{fig:architecture-of-transformer}}
\end{figure}

\subsubsection{\textbf{Graph neural networks}}

A Graph Neural Network (GNN) is a powerful deep learning architecture designed to analyze and process data represented in the form of graphs. GNNs are specialized in capturing complex relationships and interactions within interconnected nodes. They operate by propagating information through the graph's nodes and edges, allowing them to learn patterns and features from both local and global contexts. GNNs have found applications in diverse fields such as social network analysis, recommendation systems, molecular chemistry, and spatial data analysis, demonstrating their versatility in addressing real-world problems involving interconnected data points.

A graph is represented as $G=(V, E)$ where $V$ is the set of vertices (or nodes), and $E$ is the set of edges. Let $v_i \in V$ to denote a node and $e_{ij} = (v_i, v_j) \in E$ to denote an edge pointing from $v_i$ to $v_j$. The neighborhood of a node $v$ is defined as $N(v) = \{u \in V | (u, v) \in E \}$. The adjacency matrix $A$ is a $n \times n$ matrix with $A_{ij}=1$ if $e_{ij} \in E$ and $A_{ij}=0$ if $e_{ij} \notin E$. A graph may have node attributes $X$, where $X \in R^{n \times d}$ is a node feature matrix with $x_v \in R^{d}$ representing the feature vector of a node $v$. Meanwhile, a graph may have edge attributes $X^e$, where $X^e \in R^{m \times c}$ is an edge feature matrix with $x_{v,u}^{e}\in R^{c}$ representing the feature vector of an edge $(v, u)$.

One popular category of GNNs is Convolutional graph neural networks (ConvGNNs) which generalize the operation of convolution from grid data to graph data. The main idea is to generate a node $v$’s representation by aggregating its own features $x_v$ and neighbors’ features $x_u$, where $u \in N(v)$. Particularly, ConvGNNs stack multiple graph convolutional layers to extract high-level node representations. ConvGNNs play a central role in building up many other complex GNN models. Figure \ref{fig:architecture-of-ConvGNN} shows a ConvGNN with multiple graph convolutional layers for nodes' representation learning.

We consider a multi-layer Graph Convolutional Network (GCN) with the following layer-wise propagation rule:

\[
H^{(l+1)}=\sigma(\tilde{D}^{-1/2}\tilde{A}\tilde{D}^{-1/2}H^{(l)}W^{(l)})
\]

Here, $\tilde{A}=A+I_{N}$ is the adjacency matrix of the undirected graph $G$ with added self-connections. $I_{N}$ is the identity matrix,
$\tilde{D}_{ii}=\sum_{j}\tilde{A}_{ij}$ and $W^{(l)}$ is a layer-specific trainable weight matrix. $\sigma(.)$ denotes an activation function, such as the $RELU(.)=max(0,.)$. $H^{(l)}\in R^{N\times D}$ is the matrix of activations in the $l^{th}$ layer with $H^{(0)}=X$.

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.88\columnwidth]{figures/ConvGNN.png}
\par\end{centering}
\caption{A ConvGNN with multiple graph convolutional layers. A graph convolutional layer captures the underlying representation of each node by aggregating feature information from its neighborhood nodes. Following this aggregation, a non-linear transformation is applied to the resulting outputs. By stacking multiple layers, the final representation of each node receives messages from its neighborhood. \label{fig:architecture-of-ConvGNN}}
\end{figure}

Please refer to \cite{GNNssurveys} for the details of other categories of graph neural networks (GNNs) including Recurrent graph neural networks (RecGNNs), Graph autoencoders (GAEs), and Spatial-temporal graph neural networks (STGNNs).

\subsubsection{\textbf{Mahalanobis distance}}

A rich line of machine learning and deep learning algorithms has been developed for out-of-distribution (OOD) detection, among which distance-based methods demonstrated promise \cite{lee2018simple, Tack2020, Sehwag21}. Distance-based methods leverage feature embeddings extracted from a model and operate under the assumption that the test OOD samples are relatively far away from the ID data. For example, \cite{Sehwag21} uses the Mahalanobis distance \cite{Mahalanobis} to all cluster centroids for OOD detection. In particular, the authors first partition the features for in-distribution training data in $M$ clusters. They represent features for each cluster as $Z_m$ (by using the k-means clustering method due to its effectiveness and low computation cost). Next, they model features in each cluster independently and calculate the following $outlier\, score(s_{\mathbf{x}})=min_{m}D(\mathbf{x}, Z_{m})$ for each test input $\mathbf{x}$, where $D(., .)$ is a distance metric in the feature space. The Mahalanobis distance to calculate the outlier score of each input data $x$ in the latent space is as follows:

\[
s(x)=min_{k}(\mathbf{z}_\mathbf{x}-\mu_{m})^{\mathrm{\top}}\Sigma_{m}^{-1}(\mathbf{z}_\mathbf{x}-\mu_{m})
\]

where $\mathbf{z}_\mathbf{x}$ is the representation of data $\mathbf{x}$ in the latent space while $\mu_{m}$ and $\Sigma_{m}$ are the sample mean and sample covariance of cluster $m^{th}\in M$.

\subsubsection{\textbf{Contrastive loss functions}}

Using contrastive loss functions for improving data representations has been widely applied to computer vision domain applications from computer vision classification, detection, and segmentation \cite{NEURIPS2020_Kim, Wang_2021_ICCV, Sun_2021_CVPR, Du_2022_CVPR, Wang_2021_CVPR} to vision data out-of-distribution detection \cite{Sehwag21}.

\paragraph{\textbf{Self-supervised contrastive learning}}

For a set of $N$ randomly sampled sample and label pairs, $\{\mathbf{x}_k, y_k\}_{k=1...N}$, the corresponding batch used for training consists of $2N$ pairs, $\{\tilde{\mathbf{x}}_l, \tilde{y}_l\}_{l=1...2N}$, where $\tilde{\mathbf{x}}_{2k}$ and $\tilde{\mathbf{x}}_{2k-1}$ are two random augmentations of $\mathbf{x}_k (k=1...N)$ and $\tilde{y}_{2k-1}=\tilde{y}_{2k} = y_k$. We refer to a set of $N$ samples as a “batch” and the set of 2N augmented samples as a “multi-viewed batch”.

Within a multi-viewed batch, let $i\in I \equiv \{1...2N\}$ be the index of an arbitrary augmented sample, and let $j(i)$ be the index of the other augmented sample originating from the same source sample.
In self-supervised contrastive learning (SimCLR), the loss takes the following form:

\[
\mathcal{L}^{self}=\sum_{i\in I}\mathcal{L}_{i}^{self}=-\sum_{i\in I}log\frac{exp(sim(\mathbf{z},\mathbf{z}_{j(i)})/\tau)}{\sum_{\alpha\in A(i)}exp(sim(\mathbf{z},\mathbf{z}_{a})/\tau)}
\]

where $\mathbf{z}_{l}$ can be considered as a representation of corresponding $\mathbf{x}$; $sim$ function can be the inner (dot) product; $\tau\in R^{+}$ is a scalar temperature parameter, and $A(i) \equiv I\setminus{i}$. The index $i$ is called the anchor, index $j(i)$ is called the positive, and the other $2(N-1)$ indices ($\{k \in A(i) \setminus \{j(i)\}\})$ are called the negatives. Note that for each anchor $i$, there is one positive pair and $2N-2$ negative pairs. The denominator has a total of $2N-1$ terms (the positives and negatives).

\paragraph{\textbf{Supervised contrastive learning}}
Supervised contrastive learning (SupCLR) is a supervised version of self-supervised contrastive learning (SimCLR). That builds on the contrastive self-supervised literature by leveraging label information. Normalized embeddings from the same class are pulled closer together than embeddings from different classes:

\[
\mathcal{L}^{sup}=\sum_{i\in I}\mathcal{L}_{i}^{sup}=\sum_{i\in I}\frac{-1}{\left|P(i)\right|}log\frac{exp(sim(\mathbf{z},\mathbf{z}_{p})/\tau)}{\sum_{\alpha\in A(i)}exp(sim(\mathbf{z},\mathbf{z}_{a})/\tau)}
\]

where $P(i) \equiv \{p \in A(i): \tilde{y}_p = \tilde{y}_i\}$ is the set of indices of all positives in the multi-viewed batch distinct from $i$, and $\left|P(i)\right|$ is its cardinality.

\subsubsection{\textbf{Cosine similarity}}\label{sec:cosines}

Cosine similarity is a metric used to measure the similarity of two vectors. In particular, cosine similarity measures the similarity in the direction or orientation of the vectors ignoring differences in their magnitude or scale. The similarity of two vectors is measured by the cosine of the angle between them (please refer to Figure \ref{fig:cosine-similarity} for details). In our paper, to form the corresponding vector for each $\tilde{X}$ of each source code section $X$ in the latent space for calculating the cosine similarity, we simply concatenate all vectors where each vector stands for a representation of a code statement in $\tilde{X}$.

\subsection{\textbf{Mutual information}}

Mutual information (MI) is used to measure the dependence
between two random variables \cite{TheoryofC, EofIT2006}. It captures how much the knowledge of one random variable reduces the uncertainty of the other. In particular, MI quantifies the amount of information obtained about one random variable by observing the other random variable. For instance, suppose variable A signifies the outcome of rolling a standard 6-sided die, and variable B represents whether the roll yields an even (0 for even, 1 for odd) result. It is evident that information from B offers insights into the value of A, and vice versa. In essence, these random variables exhibit mutual information.

Assume that we have two random variables $X$ and $Y$ drawn from the joint distribution $p(x,y)$ with two corresponding marginal distributions $p(x)$ and $p(y)$. The mutual information between $X$ and $Y$ denoted by $I(X,Y)$ is the relative entropy between the joint distribution $p(x,y)$ and the product distribution $p(x)p(y)$, and is defined as follows:

\vspace{-1mm}
%\[
%I(X,Y)=\sum_{x\in\mathcal{X}}\sum_{y\in\mathcal{Y}}p(x,y)\log\frac{p(x,y)}{p(x)p(y)}=D_{KL}(p(x,y)||p(x)p(y))
%\]

\begin{align*}
I(X,Y) & =\int p(x,y)\log\frac{p(x,y)}{p(x)p(y)}dxdy\\
 & =D_{KL}(p(x,y)||p(x)p(y))
\end{align*}

\vspace{1mm}
where $D_{KL}(p(x,y)||p(x)p(y))$ is the Kullback-Leibler divergence measuring the relative entropy (i..e, the difference in information) represented by two distributions, i.e., the product of marginal distributions $p(x)p(y)$ of $X$ and $Y$ from their joint distribution $p(x,y)$.

\subsubsection{\textbf{Information bottlenecks}}

Here, we consider the supervised learning context where we want to predict corresponding outputs (e.g., labels) $\left\{ \by_{i}\right\} _{i=1}^{n}$ of given inputs $\left\{ \bx_{i}\right\} _{i=1}^{n}$. A deep learning network (DNN) will learn latent representations (i.e., latent features in the latent space that contain useful information to describe the data) $\left\{ \tilde{\bx}_{i}\right\} _{i=1}^{n}$ of the corresponding input data samples $\left\{ \bx_{i}\right\} _{i=1}^{n}$ in terms of enabling good predictions and generalizations.

Assume that the whole hidden layer in Figure \ref{fig:Bottneck_theory} is denoted by a random variable $\tilde{X}$ while the input and output layers are denoted by random variables $X$ and $Y$ respectively. We can describe this hidden layer by two conditional distributions: the encoder $p(\tilde{\bx}|\bx)$ and the decoder $p(\by|\tilde{\bx})$. This transformation process preserves the information of the input layer $X$ without considering which individual neurons within the hidden layer $\widetilde{X}$ encode which features (i.e., neurons) of $X$. An optimal encoder process of the mutual information between $X$ and the desired output $Y$ denoted by $I(X,Y)$ can create the most compact encoding (i.e., minimally sufficient statistic) $\tilde{X}$ of the input data $X$ while $\tilde{X}$ still has enough information (i.e., $\tilde{X}$ can capture the important features of $X$ as well as remove the unnecessary parts of $X$ that do not make any contributions to the prediction of $Y$) to predict $Y$ as accurately as possible.

An information bottleneck \cite{tishby2000information,tishby2015deep}
is proposed to be a computational framework that aims to find the most compact encoding $\tilde{X}$ of the input data $X$. In particular, it is the optimal trade-off between the compression $\tilde{X}$ and the prediction of the desired output $Y$ as described in the following optimization problem:
\begin{equation}
\min_{p(\tilde{\bx}|\bx),p(\by|\tilde{\bx}),p(\tilde{\bx})}\left\{ I(X,\tilde{X})-\beta I(\tilde{X},Y)\right\} \label{eq:information-bottleneck}
\end{equation}

where $\beta$ specifies the amount of relevant information captured by the encoding process (i.e., the representations $\tilde{X}$ and $I(\tilde{X}, Y)$).

\begin{figure}[h]
\begin{centering}
\includegraphics[width=0.5\columnwidth]{figures/Bottleneck_theory.pdf}
\par\end{centering}
\vspace{-1mm}
\caption{An architecture of a simple deep neural network in a supervised learning context for the classification problem. \label{fig:Bottneck_theory}}
\end{figure}

\begin{figure*}[t]%
\begin{centering}
%\vspace{-1mm}
\begin{tabular}{c}
\includegraphics[width=0.9\textwidth]{figures/Cosine_similarity_v2.pdf}\tabularnewline
\end{tabular}\vspace{-1mm}
\par\end{centering}
\caption{A graphic showing two vectors with cosine similarities close to 1, close to 0, and close to -1. The similarity of two vectors is measured by the cosine of the angle between them. The similarity can take values between -1 and +1. Smaller angles between vectors produce larger cosine values, indicating greater cosine similarity.\label{fig:cosine-similarity}}
\vspace{-3mm}
\end{figure*}%

==> sections/related_work_sup.tex <==
\section{Related Work}\label{sec:related_work}

\subsection{\textbf{OOD data identification}}

There have been many AI-based methods (i.e., machine learning-based and deep learning-based approaches) introduced for out-of-distribution detection widely applied to computer vision and medical diagnosis applications. While traditional methods, e.g., one-class SVMs \cite{Scholkopf1999}, have been revisited with deep representations \cite{pmlr-v80-ruff18a}, yielding improvements to complex data, the vast majority of deep learning existing efforts toward developing efficient detection solutions have studied threshold-based detectors \cite{HendrycksG16c, LiangLS17, GuoPSW17, Lakshminarayanan-2016} using the confidence (or entropy) of the predictive distribution $p(Y|X)$ (where $Y$ denotes the label of the corresponding data $X$) of (or assembles of) discriminative classifiers trained on in-distribution data. Lee et al.\cite{Lee18a} and Hendrycks et al. \cite{Hendrycks18} further introduced confidence losses that use an auxiliary dataset (i.e., a generative adversarial network (GAN) \cite{goodfellow-2014} for generating the most effective samples from $P_{out}$ (out-of-distribution) or a dataset entirely disjoint from test-time data) to teach the network better representations for anomaly detection. Lee et al. \cite{Lee18b} proposed a method that is applicable to any pre-trained softmax neural classifier (without re-training) for detecting abnormal test samples including OOD and adversarial ones. In particular, the idea is to measure the probability density of the test sample on feature spaces of DNNs utilizing the concept of a generative (distance-based) classifier. 

Recently, Hendrycks et al. \cite{Hendrycks2019} proposed a method using self-supervised learning with image rotation prediction for enabling the detection of out-of-distribution examples while Winkens et al. \cite{Winkens2020} introduced a contrastive training (in addition to supervised classification losses) on image data for out-of-distribution detection. Sehwag et al. \cite{Sehwag21} proposed an outlier detector using self-supervised representation learning \cite{TingChen-2020, YonglongTian-2020} followed by a Mahalanobis distance-based detection in the feature space.

An alternative for out-of-distribution detection is to use generative model-based methods, which are appealing as they do not require labeled data and can directly model the input data distribution. Specifically, these methods fit a generative model 
to the input data and then evaluate the likelihood of new inputs under that model. However, some later works (e.g., \cite{Nalisnick18} and \cite{Choi18}) have highlighted significant issues with this approach for OOD detection on images, showing that deep generative models such as Glow \cite{Kingma18} and PixelCNN \cite{OordKK16, SalimansKCK17} sometimes assign higher likelihoods to OOD than in-distribution inputs. Ren et al. \cite{Ren19} proposed a likelihood ratio method that uses a background model to correct the background statistics and enhances the in-distribution specific features for OOD detection applied to images and genomics sequences data.


Although most of the existing methods have achieved promising results for out-of-distribution detection,  they are mainly based on or only applicable to computer vision applications or medical diagnosis. Automated deep learning-based techniques for out-of-distribution source code data identification have not yet been well studied. \revise{\textit{In our paper, we apply some state-of-the-art out-of-distribution detection methods (e.g., \cite{Hendrycks2017dnn, Hendrycks18, Sehwag21}) to the problem of identifying OOD source code data, and we compare the performance of these models to our proposed method} (please refer to the Experiment section (Section \ref{sec:experiments}) for details)}.

\subsection{\textbf{Software vulnerability detection}}

AI-based approaches have been proposed for software vulnerability detection (SVD). Most previous work in SVD, such as \cite{yamaguchi2011vulnerability, shin2011evaluating, Li2016:VAV, Grieco2016, KimWLO17}, was based primarily on handcrafted features manually chosen by knowledgeable domain experts with possibly outdated experience and underlying biases. In many situations, these handcrafted features do not generalize well. For example, features that work well in a certain software project may not perform well in other projects \cite{Zimmermann2009}. To alleviate the dependency on handcrafted features, the use of automatic features in SVD has been studied recently \cite{VulDeePecker2018,jun_2018, Dam2018, Li2018SySeVR, Duan2019, Cheng2019, Zhuang2020, ReGVD2022, nguyen2022info, nguyen2022cross}. These methods show the advantages of employing automatic features over handcrafted features for SVD. 

Although achieving significant performances in many domain applications (e.g., autonomous driving, biometric authentication, and cyber security), AI-based methods are well-known to fail against the input data lying far away from the training data distributions. \revise{\textit{In our paper, we want to investigate if effective methods in SVD can produce a good performance on identifying out-of-distribution CWE source code data. In particular, we evaluate the capability of these models to accurately discern whether an input data sample originates from an out-of-distribution category.}}

Therefore, additional baselines of our proposed method are some effective and state-of-the-art methods for software vulnerability detection including \cite{VulDeePecker2018, ReGVD2022, CodeBERT2020}. \textbf{VulDeePecker} \cite{VulDeePecker2018} is considered one of the most effective deep learning-based software vulnerability detection methods leveraging the power of bi-directional long-short-term memory (LSTM) networks. \textbf{CodeBERT} \cite{CodeBERT2020} is a pre-trained model (based on the Transformer's encoder framework \cite{transformers-Vaswani17}) that specializes in the programming language. Via CodeBERT, we aim to investigate how large language models work in the context of out-of-distribution source code data identification. \textbf{ReGVD} \cite{ReGVD2022} is a simple yet effective graph neural network-based model for the software vulnerability detection problem.

\subsection{The difference between source code vulnerability detection and OOD source code identification tasks}

\revise{It is important to note that the task of identifying out-of-distribution source code data differs from that of source code vulnerability detection. In the out-of-distribution identification task, we solely aim to detect if input data is from an established in-distribution or out-of-distribution category while in the vulnerability detection, we aim to detect the vulnerability (e.g., vulnerable or non-vulnerable) of the data.} The out-of-distribution stage assists the security system in identifying out-of-distribution source code data (that can be vulnerable or benign) outside the established in-distribution data before feeding input data into subsequent machine learning and deep learning modules, including the vulnerability detection phase.

==> sections/supp_experiments.tex <==
\section{Experiments}

\subsection{\textbf{Data processing and embedding}}

We preprocessed the datasets before injecting them into our proposed \ourapp~method and baselines. In particular, we standardized the source code data samples by (i) removing comments, blank lines, and non-ASCII characters, and (ii) mapping user-defined variables to symbolic variable names (e.g., \emph{var1} and \emph{var2}) and user-defined
functions to symbolic function names (e.g., \emph{func1} and \emph{func2}) using Treesitter \cite{Treesitter}.  We also replaced strings with a generic \emph{"str"} token.

We then embedded source code statements into vectors. For instance, consider the following statement (written in C/C++ programming language) \textit{for(var1=0;var1$<$10;var1++}, we tokenize this statement into a sequence of tokens (i.e., \textit{for,(,var1,=,0,;,var1,$<$,10,;,var1,++,)}), and then we used a 150-dimensional Embedding layer followed by a Dropout layer (with a dropped fixed probability $p=0.2$), a 1D convolutional layer (with the filter size $150$ and kernel size $3$), and a 1D max pooling layer to encode each source code statement in a source code function $X$. Note that we utilize the commonly used values for these hyperparameters. Finally, a mini-batch of functions in which each function consisting of $L$ encoded statements was fed to the deep learning-based models. It is worth noting that the Embedding and 1D convolutional layers are learnable during the training process.

It is worth noting that from the used datasets, the length ($L$) of each function is padded or truncated to $100$ source code statements  (i.e., we base on the quantile values of the source code data’ length to decide the length of each source code data sample). Specifically, more than 95\% of the functions consist of 100 or fewer source code statements. Furthermore, we observe that almost all important information relevant to the vulnerability of each source code data sample (e.g., a function) lies in the first $100$ source code statements.

\subsection{\textbf{A summary of the baselines}}

We briefly summarize the baselines as follows:
\begin{itemize}
    \item \textbf{Standard DNN} \cite{Hendrycks2017dnn}. It is a baseline utilizing probabilities from softmax distributions for detecting misclassified and out-of-distribution examples in neural networks.\vspace{1mm}
    \item \textbf{Outlier Exposure} \cite{Hendrycks18}. It enables OOD (anomaly) detectors to generalize and detect unseen anomalies by training anomaly detectors against an auxiliary dataset of outliers disjoint from the testing dataset (i.e., OOD data).\vspace{1mm}
    \item \textbf{SSD} \cite{Sehwag21}. An outlier detector method utilizes contrastive representation learning followed by a Mahalanobis distance-based detection in the feature space for outlier (out-of-distribution) detection.\vspace{1mm}
    \item \textbf{VulDeePecker} \cite{VulDeePecker2018}. It is one of the most effective deep learning-based software vulnerability detection methods leveraging the power of bi-directional long-short-term memory (LSTM) networks \cite{hochreiter1997long-short}.\vspace{1mm}
    \item \textbf{CodeBERT} \cite{CodeBERT2020}. A pre-trained model (based on the Transformer's encoder framework \cite{transformers-Vaswani17}) specializes in the programming language. Via CodeBERT, we aim to investigate how large language models work in the context of out-of-distribution source code data identification.\vspace{1mm}
    \item \textbf{ReGVD} \cite{ReGVD2022}. It is an effective Graph neural network-based model (i.e., using Graph convolutional networks \cite{GCNN2017} and Gated graph neural networks \cite{Gated2016}) for the software vulnerability detection problem.
\end{itemize}

\subsection{\textbf{Model's configurations}}

For the main baselines of our \ourapp~method including Standard DNN \cite{Hendrycks2017dnn}, Outlier Exposure \cite{Hendrycks18}, and SSD \cite{Sehwag21}. These methods are popular and state-of-the-art approaches for out-of-distribution detection applied in the computer vision domain. To make them applicable for out-of-distribution source code vulnerability detection, we keep the principle of these methods and use the same data embedding process for handling the sequential source code data as used in our method. For the additional baseline approaches, popular and state-of-the-art SVD methods (i.e., VulDeePecker \cite{VulDeePecker2018}, CodeBERT \cite{CodeBERT2020}, and ReGVD \cite{ReGVD2022}), we use the architecture proposed in the corresponding original papers.

To our \ourapp~method, for the $g\left(\cdot;\alpha\right)$
and $f\left(\cdot;\beta\right)$ networks, we used deep feed-forward neural networks having three and two hidden layers with the size of each hidden layer in $\left\{100,300\right\} $. The dense hidden layers are followed by a ReLU function as nonlinearity and Dropout \cite{srivastava14a} with a retained fixed probability $p=0.8$ as regularization. The last dense layer of the $g\left(\cdot;\alpha\right)$ network for learning a discrete distribution is followed by a sigmoid function while the last dense layer of the $f\left(\cdot;\beta\right)$ network is followed by a softmax function for predicting. The number of chosen clusters guiding the computation of the innovative cluster-contrastive learning mentioned is set in $\{1, 3, 5, 7, 9\}$. The trade-off hyper-parameter $\lambda$ representing the weight of the innovative cluster-contrastive learning is in $\{10^{-2},10^{-1},10^{0}\}$ while the scalar temperature $\tau$ is in $\{0.5, 1.0\}$. The temperature $\nu$ for the Gumbel softmax distribution is also set in $\{0.5, 1.0\}$. Note that we utilize
the commonly used values for these hyperparameters.

For our \ourapp~method and baselines, we employed
the Adam optimizer \cite{KingmaB14} with an initial learning rate equal to $10^{-3}$, while the mini-batch size is set to $128$. For the training process, we split the data of each in-distribution data into two random partitions. The first partition contains 80\% for training, the second partition contains 20\% for validation. For each in-distribution data, we used $10$ epochs for the training process. We additionally applied gradient clipping regularization to prevent over-fitting. For each method, we ran the corresponding model several times and reported the averaged FPR (at TPR 95\%), AUROC, and AUPR measures. We ran our experiments in Python using Tensorflow \cite{abadi2016tensorflow} for the used methods on a 13th Gen Intel(R) Core(TM) i9-13900KF having 24 CPU Cores at 3.00 GHz with 32GB RAM, integrated Gigabyte RTX 4090 Gaming OC 24GB. Some baseline methods (i.e., CodeBERT \cite{CodeBERT2020} and ReGVD \cite{ReGVD2022}) were written using Pytorch \cite{pytorch2019}. For these baselines, we followed the source code samples published by the authors.

\input{sections/discussion}

\subsection{\textbf{Additional experiments}}
Here we present some additional experiments of our \ourapp~method and baselines on other further cases of the in-distribution (ID) and out-of-distribution (OOD) CWE source code data categories. The experimental results in Table \ref{tab:my_label_app} again show the effectiveness and superiority of our proposed \ourapp~method compared to the baselines for out-of-distribution source code data identification by a wide margin. Notably, in these additional cases, on average, our LEO method obtains a significantly higher performance from around 10.59\%, 4.65\%, and 6.72\% on the FPR, AUROC, and AUPR measures, respectively, in comparison with the baselines.

\input{tables/table2app}


==> sections/supp_frameworks.tex <==
\section{The proposed \ourapp~approach}\label{sec:framework}

\vspace{1mm}
\subsection{\textbf{The selection of important source code statements}}

As depicted in Figure 1 (in the main paper), our \ourapp~method starts with a selection network $\zeta$ for automatically learning and figuring out the crucial and \revise{label-relevant code statements} in each source code data (a function or a program). It is important to highlight that to vulnerable source code data, the identified code statements constitute the corresponding vulnerability patterns, rendering the data vulnerable. Through the selection network with the use of innovative cluster-contrastive learning, in the latent space, the source code data containing different hidden vulnerability patterns will be trained to have different representations, causing them to be situated far apart from each other while the source code data sharing similar hidden vulnerability patterns are encouraged to remain closely clustered. This process elegantly facilitates \revise{out-of-distribution source code data identification.}

\paragraph{\textbf{Reparameterization for continuous optimization}}
To make the selection process (i.e., the process consists of sampling operations from a Multi-Bernoulli distribution) continuous and differentiable during training, we apply the Gumbel-Softmax trick {\cite{jang2016categorical, MaddisonMT16}} for relaxing each Bernoulli variable $z_{i}$. Specifically, we sample $z_{i}\left(X;\alpha\right)\sim\text{Concrete}(g_{i}(X;\alpha),1-g_{i}(X;\alpha))$:

\vspace{-5mm}
\begin{align*}
& z_{i}\left(X;\alpha\right)\\
 = & \frac{\exp\{(\log g_{i}+a_{i})/\nu\}}{\exp\{(\log g_{i}+a_{i})/\nu\}+\exp\{(\log\left(1-g_{i}\right)+b_{i})/\nu\}}
\end{align*}
\vspace{-2mm}

where we denote $g_{i}\left(X;\alpha\right)$ as $g_{i}$ while $\nu$ is a temperature parameter (i.e., controlling how closely a continuous representation from a Gumbel-Softmax distribution approximates this from the corresponding discrete representation from a discrete distribution (e.g., the Bernoulli distribution)), random noises $a_{i}$ and $b_{i}$ independently drawn from \textbf{Gumbel} distribution
$G = - \log(- \log u)$ with $\ u \sim \textbf{Uniform}(0,1)$.

\subsection{\textbf{The algorithm of the proposed \ourapp~method}}

Algorithm 1 exhibits the details of our LEON method in both
the training and testing phases.

\RestyleAlgo{ruled}
\begin{algorithm*}[htbp]
\vspace{1mm}
\input{sections/algorithm}\caption{The algorithm of our proposed \ourapp~method for out-of-distribution source code identification.\label{alg:The-training-algorithm-prom}}
\vspace{0mm}
\end{algorithm*}

\vspace{3mm}

==> tables/table1t_details.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.93\columnwidth}{!}{
%{|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 
%\hline		

{CWE287 vs. CWE416}
 &  Standard DNN & 86.30\%	& 67.93\% & 84.60\% 
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  79.30\%	& 68.93\% & 86.13\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 84.78\%	& \underline{66.71\%} & 84.67\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{77.63\%}	& 68.20\% & \underline{85.61\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT &  88.57\% & 68.25\% & 85.49\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD &  90.40\%	& 58.58\% & 81.88\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

   & {\ourapp~ (Ours)} & \textbf{69.71\%} & \textbf{76.75\%} & \textbf{90.57\%}\tabularnewline
 
\hline 
%\hline 	
 
{CWE269 vs. CWE200}
 &  Standard DNN & 79.36\%	& 69.28\%	& 78.75\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  80.30\%	& 70.05\%	& 78.49\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 79.92\%	& 72.70\%	& 78.86\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{83.90\%}	& \underline{74.73\%}	& \underline{81.62\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 88.43\%	& 65.64\%	& 74.55\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 93.74\%	& 61.01\%	& 69.55\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO (Ours)} & \textbf{76.89\%} & \textbf{79.33\%} & \textbf{85.32\%}\tabularnewline
 
 \hline
 %\hline
 
{CWE863 vs. CWE862}
 &  Standard DNN & 77.42\%	&  81.36\%	&  57.53\% 
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  77.42\%	&  83.83\%	&  62.19\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 61.29\%	&  75.95\%	&  66.83\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{77.42\%}	&  \underline{83.11\%}	&  55.39\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT  &  76.67\%	& 68.85\%	&  \underline{48.24\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  &  96.67\%	&  66.95\%	&  37.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO (Ours)} & \textbf{54.84\%} & \textbf{84.31\%} & \textbf{70.76\%}\tabularnewline
 
 \hline
 %\hline 	
 
{CWE94 vs. CWE20}
 &  Standard DNN & \underline{73.26\%}	& 75.60\%	& 95.60\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  74.44\%	& 75.83\%	& 95.28\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 85.70\%	& \underline{70.40\%}	& \underline{94.17\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & 77.85\%	& 73.79\%	& 95.54\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 87.55\%	& 74.93\%	& 94.58\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 94.74\%	& 66.98\%	& 92.55\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

  & {LEO (Ours)} &  \textbf{51.70\%}	& \textbf{84.37\%} & \textbf{97.72\%}\tabularnewline
 
\hline 	
 
{CWE190 vs. CWE119}
&  Standard DNN & 85.54\%	& 69.97\%	& 60.47\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure &  82.69\%	& 69.93\% & 60.22\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 77.87\%	& \underline{74.46\%}	& \underline{66.04\%}
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 85.17\%	& 70.01\%	& 59.79\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 90.72\%	& 68.74\%	& 55.74\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD & \underline{96.66\%}	& 50.50\%	& 41.33\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

&  {\ourapp~ (Ours)}  & \textbf{68.85\%} & \textbf{77.59\%} & \textbf{72.42\%}
\tabularnewline
\hline	
 
{CWE269 vs. CWE20}
 &  Standard DNN & 72.96\%	& 71.90\%	& 91.43\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  77.33\%	& 73.29\%	& 91.62\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 85.33\%	& 69.69\%	& 89.44\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{79.63\%}	& \underline{71.23\%}	& \underline{903.3\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 91.40\%	& 67.44\%	& 87.62\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD & 92.51\%	& 62.60\%	& 86.31\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO (Ours)} & \textbf{64.30\%} & \textbf{79.51\%} & \textbf{93.95\%}\tabularnewline
 
 \hline
%\hline
 
\hline
\end{tabular}}
\vspace{-2mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each out-of-distribution (OOD) vulnerability corresponding with specific in-distribution (ID) data.  (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method over the second-best values from the baselines.)}\label{tab:my_label1t}
\vspace{-2mm}
\end{table}



==> tables/table23t_details.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.93\columnwidth}{!}{
% {|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 
 
& StandardDNN & 54.55\%	& 80.00\%	& 64.71\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  57.58\%	& 80.68\%	& 65.78\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE863-862}
 &  SSD & 48.48\%	& 89.22\%	& 71.28\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE287}
 &  VulDeePecker & \underline{60.61\%}	& \underline{82.48\%}	& \underline{56.61\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 63.08\%	& 89.60\%	& 64.08\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 83.33\%	& 67.89\%	& 39.98\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} &  \textbf{37.88\%}	& \textbf{90.48\%} & \textbf{78.69\%}\tabularnewline
 
\hline 
%\hline 
 
& StandardDNN & 81.48\%	& 73.10\% & 86.88\% 
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  75.41\%	& 75.52\% & 88.55\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE269-94}
 &  SSD & 71.70\% & 75.99\% & 89.33\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE20}
 &  VulDeePecker & \underline{79.26\%}	& \underline{73.30\%} & \underline{86.93\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT &  85.47\% & 69.37\% & 84.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD &  90.40\%	& 62.13\% & 74.91\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

& {LEO(Ours)} & \textbf{63.26\%} & \textbf{82.44\%} & \textbf{91.74\%}\tabularnewline
\hline 
%\hline 
 
& StandardDNN & 83.41\%	& 70.26\%	& 78.50\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  OutlierExposure &  86.30\%	& 67.15\%	& 77.00\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE287-94}
 &  SSD & 72.45\%	& 80.50\%	& 86.84\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE416}
 &  VulDeePecker & \underline{85.08\%}	& \underline{65.27\%}	& \underline{76.64\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 84.60\%	& 63.47\%	& 74.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 90.72\%	& 57.38\%	& 69.68\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{60.88\%} & \textbf{81.00\%} & \textbf{88.12\%}\tabularnewline
 \hline
 %\hline	
 
& StandardDNN & 80.44\%	& 73.22\%	& 91.77\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  80.07\%	& 72.59\%	& 91.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE200-125}
 &  SSD & 70.30\%	& 80.70\%	& 94.27\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
vs. {CWE264}
 &  VulDeePecker & 78.37\%	& 75.01\%	& 92.39\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & \underline{85.92\%}	& \underline{74.23\%}	& \underline{91.37\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 89.40\%	& 62.29\%	& 83.87\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{47.85\%} & \textbf{88.76\%} & \textbf{97.16\%}\tabularnewline

 \hline

& StandardDNN & \underline{84.02\%}	& \underline{67.47\%}	& 70.30\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  87.82\%	& 66.34\%	& 69.24\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE287-862-94}
 &  SSD & 71.08\%	& 74.95\%	& 78.97\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
vs. {CWE416}
 &  VulDeePecker & 78.39\%	& 67.86\%	& 72.03\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 91.62\%	& 68.64\%	& \underline{67.69\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 94.22\%	& 55.55\%	& 58.82\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{55.71\%} & \textbf{84.98\%} & \textbf{86.59\%}\tabularnewline

 \hline
\end{tabular}}
\vspace{-2mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each out-of-distribution (OOD) vulnerability corresponding with specific in-distribution (ID) data. (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method over the second-best values from the baselines.)}\label{tab:my_label23t}
\vspace{-2mm}
\end{table}


==> tables/table2app_details.tex <==
\begin{table}[ht]
\centering{}
\resizebox{0.93\columnwidth}{!}{
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD Datasets} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$& \textbf{AUROC} $\uparrow$& \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 	
 
&  StandardDNN & 50.00\%	& 80.28\%	& 78.26\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  OutlierExposure & 71.21\% &  79.29\% &  76.57\%  
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 46.97\%	& 82.55\%	& 83.78\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & \underline{48.48\%}	& \underline{79.20\%}	& \underline{76.53\%}
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 53.85\%	& 78.54\%	& 78.43\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD & 66.15\%	& 80.42\%	& 77.84\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

&  {LEO(Ours)}  & \textbf{33.33\%} & \textbf{87.06\%} & \textbf{85.99\%}
\tabularnewline
\hline	
 
&  StandardDNN & 85.14\%	& 68.41\%	& 54.78\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  OutlierExposure &  83.36\%	& 69.46\%	& 56.76\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 84.70\%	& 71.02\%	& 57.76\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & \underline{85.74\%}	& \underline{69.51\%}	& \underline{56.58\%}
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 93.01\%	& 66.19\% & 47.95\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 96.88\%	& 49.28\%	& 37.43\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

& {LEO(Ours)} & \textbf{66.42\%} & \textbf{80.39\%} & \textbf{71.58\%}\tabularnewline
 
 \hline

&  StandardDNN & 83.33\%	& 77.51\%	& 63.73\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  OutlierExposure &  83.33\%	& 71.61\%	& 56.74\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 66.67\%	& \underline{79.70\%}	& 68.64\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 80.00\%	& 70.25\%	& 57.17\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & \underline{89.89\%}	& 62.70\%	& \underline{45.01\%}
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 93.26\%	& 63.49\%	& 44.22\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

& {LEO(Ours)}  & \textbf{61.11\%} & \textbf{79.88\%} & \textbf{70.57\%}
\tabularnewline

\hline
	
 
%\hline
&  StandardDNN & 80.49\%	& 71.59\%	& 64.71\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  OutlierExposure &  83.71\% &  72.13\% & 65.96\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 72.54\%	& 77.04\%	& 73.67\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 78.79\%	& 72.24\%	& 67.30\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & \underline{90.32\%}	& \underline{70.02\%}	& \underline{59.78\%}
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 91.27\%	& 57.50\%	& 53.21\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

&  {LEO(Ours)}  & \textbf{64.96\%} & \textbf{81.25\%} & \textbf{76.69\%}
\tabularnewline
\hline
%\hline	
 
 &  StandardDNN & 83.44\%	& \underline{70.97\%}	& 57.45\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  OutlierExposure &  83.68\%	& 69.95\%	& 56.81\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 81.83\%	& 72.19\%	& 60.47\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{82.94\%}	& 70.73\%	& \underline{56.96\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 87.75\%	& 65.71\%	& 51.50\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 97.03\%	& 48.27\%	& 35.76\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{71.32\%} & \textbf{75.76\%} & \textbf{67.59\%}\tabularnewline
 \hline
 
 &  StandardDNN & 70.97\%	& \underline{77.72\%}	& 23.14\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  OutlierExposure &  87.10\%	& 78.23\%	& 19.83\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 41.94\%	& 86.33\%	& 40.63\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{70.97\%}	& 79.12\%	& \underline{20.63\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 70.00\%	& 81.30\%	& 27.82\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 90.32\%	& 59.13\%	& 10.44\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{39.39\%} & \textbf{90.64\%} & \textbf{70.85\%}\tabularnewline

 \hline
 

 &  StandardDNN & 85.23\%	& \underline{71.03\%}	& 64.04\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  85.80\%	& 70.61\%	& 63.69\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 67.99\%	& 81.90\%	& 78.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{85.61\%}	& 70.66\%	& \underline{63.13\%}
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 82.35\%	& 74.90\%	& 67.11\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 84.47\%	& 64.56\%	& 58.98\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO(Ours)} & \textbf{54.36\%} & \textbf{84.71\%} & \textbf{82.89\%}\tabularnewline
 \hline
 
\end{tabular}}
\vspace{-1mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code samples of each out-of-distribution data with the corresponding used in-distribution data. (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method \ourapp~ over the second-best values from the baselines.)}\label{tab:my_label_app}
\vspace{-3mm}
\end{table}

==> tables/table2leo_details.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.95\columnwidth}{!}{
% {|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 

 &  \ourapp-woCD & 83.14\%	& 69.29\%	& 78.13\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 & {LEO}  &  76.89\%	& \textbf{79.33\%} & \textbf{85.32\%}\tabularnewline
 
\hline 
%\hline 

 &  \ourapp-w/oCD &  78.07\%	& 73.54\% & 95.43\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}

  & {LEO}  & \textbf{51.70\%} & \textbf{84.37\%} & \textbf{97.72\%}\tabularnewline 

\hline 
%\hline 	

& \ourapp-w/oCD & 81.13\%	& 62.99\%	& 84.96\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}

 & {LEO}  & \textbf{69.71\%} & \textbf{76.75\%} & \textbf{90.57\%}\tabularnewline
\hline
%\hline	

 &  \ourapp-w/oCD &  84.93\%	&  62.12\%	&  75.56\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}

 & {LEO}  & \textbf{60.88\%} & \textbf{81.00\%} & \textbf{88.12\%}\tabularnewline
 \hline
 %\hline 

&  \ourapp-w/oCD & 50.00\% & 79.15\%	& 62.60\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}

& {LEO}  & \textbf{37.88\%} & \textbf{90.48\%} & \textbf{78.69\%}\tabularnewline
\hline

&  \ourapp-w/oCD & 80.49\% & 70.88\%	& 65.85\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}

& {LEO}  & \textbf{54.36\%} & \textbf{84.71\%} & \textbf{82.89\%}\tabularnewline

\hline

\end{tabular}}
\vspace{-1mm}
\caption{The results of our method for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each OOD vulnerability corresponding with specific in-distribution (ID) data when using and without using the cluster-contrastive learning and the data-distribution mechanism. (The higher results for each measure in each pair of the ID and OOD data are in \textbf{bold}. The numbers highlighted in the blue color are the improvements of \ourapp~ over \ourapp-w/oCD.)}\label{tab:my_label2leo}
\vspace{-2mm}
\end{table}

==> usenix_version/sections/algorithm.tex <==
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
%\SetAlgoLined
%\SetAlgoVlined
\LinesNumbered

\KwIn{
An in-distribution source code data $D_{in}=\left\{ \left(X_{1},Y_{1}\right),\dots,(X_{N_{D_{in}}},Y_{N_{{D_{in}}}})\right\} $ where each source code data sample $X_{i}$ consisting of $L$ code statements from $\mathbf{x}_{1}$ to $\mathbf{x}_{L}$ while its vulnerability $Y_{i}\in\left\{ 0,1\right\} $ (i.e., $1$: vulnerable and $0$: non-vulnerable) will be used during the training phase. An out-of-distribution vulnerability source code data $D_{out}$ is used at the inference (testing) phase, denoted as $X_{test}$. \newline
We denote the number of training iterations $nt$; the mini-batch size $m$;
the trade-off hyper-parameter $\lambda$; and the number of clusters used in cluster-contrastive learning $K$. \newline
We randomly partition $D_{in}$ into the training set $D_{train}$ and the validation set $D_{val}$.
}
\BlankLine
We initialize the parameters $\alpha$ and $\beta$ of the selection model $\zeta$ parameterized by $g(.,\alpha)$ and the classifier model $f(.,\beta)$, respectively.
\BlankLine
\textbf{Training Phase}
\BlankLine
\For{$t=1$ to $nt$}
{
Choose a mini-batch of source code data samples denoted by $\{(X_{i},Y_{i})\}_{i=1}^{m}$.
\BlankLine
Update the classifier parameter $\beta$ via minimizing the following cross-entropy loss $\mathcal{L}_{ce}$ $E_{X,Y}E_{\mathbf{r}\sim B(0.5)}[\mathcal{L}_{ce}(Y,f_{\beta}(X\odot\mathbf{r})]$ using the Adam optimizer \cite{KingmaB14}. Note that minimizing this function is equivalent to maximizing the objective function mentioned in Eq. (\ref{eq:realx}).\;
\BlankLine
Update the classifier's parameter $\beta$ and the selection model parameter's $\alpha$ via minimizing the following objective function $E_{X,Y}E_{\mathbf{z}\sim q_{sel}(\mathbf{z}|X;\alpha)}[\mathcal{L}_{ce}(Y,f_{\beta}(X\odot\mathbf{z}))+\lambda\mathcal{L}_{ccl}]$ using the Adam optimizer. The $\mathcal{L}_{ccl}$ is described in Eq. (\ref{eq:cluster_cl}).\;
\BlankLine
}

\textbf{Note that} after the training phase, we obtain the optimal selection network for the source code data representation learning. The selection network can select the most meaningful and label-relevant source code statements, forming the vulnerability pattern to vulnerable data, for each source code data to facilitate out-of-distribution vulnerability detection.

\BlankLine
\textbf{Testing Phase}
\BlankLine
We partition $D_{train}$ into $K$ clusters. In particular, we use $k$-means to cluster the whole training data representations in the latent space into $K$ clusters equal to the number of clusters used in cluster-contrastive learning (mentioned in Eq. (\ref{eq:cluster_cl})).
\BlankLine
$\forall X_{i}\in X_{test}$ (denoted as $X_{i\_test}$). 
We use Mahalanobis distance to calculate the outlier (out-of-distribution) score for each testing data sample $X_{i\_test}$ as follows
$s(X_{i\_test})=min_{k}(\tilde{X}_{i\_test}-\mu_{k})^{\mathrm{\top}}\Sigma_{k}^{-1}(\tilde{X}_{i\_test}-\mu_{k})$
where $\mu_{k}$ and $\Sigma_{k}$ are the sample mean and sample covariance of cluster $k^{th}\in K$.
In short, $s_{X_{test}}=score(\tilde{X}_{test},\mu_{X_{train}},\Sigma_{X_{train}})$
\BlankLine
$\forall X_{i}\in X_{val}$ (denoted as $X_{i\_val}$). 
We use Mahalanobis distance to calculate the outlier (out-of-distribution) score for each validation data sample $X_{i\_val}$ as follows
$s(X_{i\_val})=min_{k}(\tilde{X}_{i\_val}-\mu_{k})^{\mathrm{\top}}\Sigma_{k}^{-1}(\tilde{X}_{i\_val}-\mu_{k})$
where $\mu_{k}$ and $\Sigma_{k}$ are the sample mean and sample
covariance of cluster $k$-th $\in K$.
In short, $s_{X_{val}}=score(G_{X_{val}},\mu_{X_{train}},\Sigma_{X_{train}})$
\BlankLine
Calculate $s_{X_{val}}$ (threshold) at $TPR=95\%$. (Note that the threshold value is chosen at $TPR=95\%$ as commonly used in almost all OOD methods)
\BlankLine
\eIf{($s(X_{i\_test})>s_{X_{val}}$)}
{
	$X_{i\_test}$ is an out-of-distribution data.
}
{
	$X_{i\_test}$ is an in-distribution data.
}
\BlankLine
\KwOut{$\forall X_{i}\in X_{test}$ (denoted as $X_{i\_test}$) whether $X_{i\_test}$ is out-of-distribution data sample.}

==> usenix_version/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we have successfully proposed an innovative deep learning-based approach for out-of-distribution source code vulnerability detection. Our \ourapp~ method derived from information theory, combined with the use of innovative cluster-contrastive learning and the data-distribution mechanism, has effectively learned the source code characteristics and figured out the semantic relationships between source code data samples (i.e., functions or programs) to boost the data representation learning facilitating the OOD vulnerability detection. The extensive experimental results on the top five popular real-world source code vulnerabilities demonstrate the effectiveness and advancement of our  \ourapp~ method compared to the state-of-the-art baselines by a wide margin.

==> usenix_version/sections/discussion.tex <==
\subsection{Discussion of Threats to Validity }\label{sec:discussion}

\paragraph{Construct Validity}
Key construct validity threats are if our assessments of the proposed method and baselines demonstrate their capability for out-of-distribution source code vulnerability detection. In the cyber security domain, by doing out-of-distribution vulnerability detection, we help security analysts and software engineers detect potential unknown vulnerability types coming in order to harden the security computer systems. To evaluate the performance of our method and baselines, we use three main common measures used in out-of-distribution detection including \textbf{FPR} (at TPR 95\%), \textbf{AUROC}, and \textbf{AUPR}.

\paragraph{Internal Validity}
Key internal validity threats are relevant to the choice of hyper-parameter settings (i.e., optimizer, learning rate, number of layers in deep neural networks, etc.). It is worth noting that finding a set of optimal hyperparameter settings of deep neural networks is expensive due to a large number of trainable parameters. To train our method, we only use the common or default values for the hyper-parameters such as using Adam optimizer, the learning rate equals $10^{-3}$, while the scalar temperature $\tau$ used in the cluster-contrastive learning and the temperature $\nu$ for the Gumbel softmax distribution are set in $\{0.5, 1.0\}$. For the number of clusters used in cluster-contrastive learning aiming to improve the data representation learning process, we use it as a hyperparameter. In our paper, we detail the hyperparameter settings (i.e., the value-tuned ranges of the hyperparameters) in the released reproducible source code to support future replication studies.

\paragraph{External Validity}
Key external validity threats include whether our proposed \ourapp~ method will generalize to other source code vulnerability types and whether they will work on other types of vulnerability datasets. We mitigated this problem by conducting our experiments on the top five popular (CWE) vulnerability types as mentioned in \cite{Bigdata2020} including CWE-119 (Improper Restriction of Operations within the Bounds of a Memory Buffer), CWE-20 (Improper Input Validation), CWE-125 (Out-of-bounds Read), CWE-200 (Exposure of Sensitive Information to an Unauthorized Actor), and CWE-264 (Permissions, Privileges, and Access Controls).



==> usenix_version/sections/experiments.tex <==
\section{Experiments}\label{sec:experiments}

\subsection{Experimental Designs}

The fundamental goal of our experiments is to evaluate our \ourapp~ method and compare it with state-of-the-art baselines for out-of-distribution source code vulnerability detection. Below, we present the research questions of our paper.

\vspace{1mm}
\textbf{(RQ1) \rqone}

For AI-based systems, being able to detect data that is out-of-distribution can be critical to maintaining safe and reliable predictions. Although achieving promising performances, current state-of-the-art out-of-distribution (OOD) methods are mostly applied to computer vision and medical diagnosis applications. Automated deep learning-based approaches for OOD detection to the source code data have not yet been well studied and explored. To this end, we propose one of the first methods for out-of-distribution source code vulnerability detection. We demonstrate that by taking into account source code characteristics and leveraging the correlations of the hidden vulnerability patterns inside and between the source code data samples, we can significantly improve the source code data representation learning for boosting out-of-distribution source code vulnerability detection.

\vspace{1mm}
\textbf{(RQ2) \rqtwo}

In reality, in-distribution source code data can consist of one or many different types of vulnerabilities. Therefore, in this research question, we investigate the performance of our proposed \ourapp~ method in various cases regarding the different number of vulnerability types (i.e., without loss of generality, we assume there are two and three different vulnerability types) existing in the in-distribution source code data and observe how the model performs compared to the baselines.

\vspace{1mm}
\textbf{(RQ3) \rqthree}

We aim to investigate the effectiveness of innovative cluster-contrastive learning (taking into account source code characteristics and semantic relationships) and the data-distribution mechanism in learning the true hidden vulnerability patterns existing in the vulnerable source code data. We prove that these terms significantly improve data representation learning, helping to boost the out-of-distribution source code vulnerability detection of the model.

\subsubsection{Studied datasets}\label{sec:studied_data_sets}

We conducted experiments on many different real-world vulnerability (CWE) types extracted from \textit{a well-known and big C/C++ dataset, namely Big-Vul} provided by \cite{Bigdata2020} which contains many types of vulnerabilities such as CWE119 (Improper Restriction of Operations within the Bounds of a Memory Buffer), CWE20 (Improper Input Validation), and CWE125 (Out-of-bounds Read). The Big-Vul data set was collected from 348 open-source Github projects from 2002 to 2019. It consists of 188,636 C/C++ source code functions spanning 91 different vulnerability types.

\textbf{In the scope of our paper, we focus on conducting our experiments on the top five popular (CWE) vulnerability types} \cite{Bigdata2020} including CWE-119 (Improper Restriction of Operations within the Bounds of a Memory Buffer with $26,497$ source code functions), CWE-20 (Improper Input Validation with $20,501$ source code functions), CWE-125 (Out-of-bounds Read with $7,717$ source code functions), CWE-200 (Exposure of Sensitive Information to an Unauthorized Actor with $8,636$ source code functions), and CWE-264 (Permissions, Privileges, and Access Controls with $12,487$ source code functions). Please refer to the appendix, Section \ref{sec:datape}, for the details of the data processing and embedding.

\vspace{-2mm}
\subsubsection{Baseline methods}

\textbf{The main baselines} of our proposed \ourapp~ method are some effective and state-of-the-art methods for out-of-distribution detection including \textbf{Standard DNN} \cite{Hendrycks2017dnn}, \textbf{Outlier Exposure} \cite{Hendrycks18}, and \textbf{SSD} \cite{Sehwag21}. These methods were originally applied to computer vision data applications. To make these methods able to be applied to the source code data, we keep the principles and make some modifications on the network for data representation learning as used in our method. There are other methods, e.g., \cite{Hendrycks2019, Winkens2020, Tack2020}, recently introduced for out-of-distribution detection. However, these methods were operated based on the nature of the vision data, so they are not applicable to the source code data.

\textit{Other additional baselines} of our \ourapp~ method are some state-of-the-art methods for software vulnerability detection (SVD) including \textbf{VulDeePecker} \cite{VulDeePecker2018}, \textbf{CodeBERT} \cite{CodeBERT2020}, and \textbf{ReGVD} \cite{ReGVD2022}. We investigate how these effective SVD methods perform for out-of-distribution vulnerability detection.

\vspace{1mm}
We briefly summarize the baselines as follows:
\begin{itemize}
    \item \textbf{Standard DNN} \cite{Hendrycks2017dnn}. It is a baseline utilizing probabilities from softmax distributions for detecting misclassified and out-of-distribution examples in neural networks.
    \item \textbf{Outlier Exposure} \cite{Hendrycks18}. It is used for enabling out-of-distribution (anomaly) detectors to generalize and detect unseen anomalies by training anomaly detectors against an auxiliary dataset of outliers disjoint from the testing dataset (i.e., out-of-distribution data).
    \item \textbf{SSD} \cite{Sehwag21}. An outlier detector method utilizes contrastive representation learning followed by a Mahalanobis distance-based detection in the feature space for outlier (out-of-distribution) detection.
    \item \textbf{VulDeePecker} \cite{VulDeePecker2018}. It is one of the most effective deep learning-based software vulnerability detection methods leveraging the power of bi-directional long-short-term memory (LSTM) networks \cite{hochreiter1997long-short}.
    \item \textbf{CodeBERT} \cite{CodeBERT2020}. A pre-trained model (based on the Transformer's encoder framework \cite{transformers-Vaswani17}) specializes in the programming language. Via CodeBERT, we aim to investigate how large language models work in the context of out-of-distribution vulnerability detection.
    \item \textbf{ReGVD} \cite{ReGVD2022}. It is an effective Graph neural network-based model (i.e., using Graph convolutional networks \cite{GCNN2017} and Gated graph neural networks \cite{Gated2016}) for the software vulnerability detection problem.
\end{itemize}

Please refer to the appendix, Section \ref{sec:modelc}, for the details of the model's configurations of our \ourapp~ method and baselines.

\vspace{-2mm}
\subsubsection{Measures}

To measure the performance of our \ourapp~ method and baselines, we use three main metrics, i.e., \textbf{FPR} (at TPR 95\%), \textbf{AUROC}, and \textbf{AUPR}, used in almost all of the out-of-distribution detection methods, notably \cite{Hendrycks18, Sehwag21}. In particular, the \textbf{FPR} (at TPR 95\%) metric calculates how many percent of out-of-distribution data are predicted as in-distribution data. \textit{For the FPR measure, the smaller value is better}. 

The \textbf{AUROC} (the area under the receiver operating characteristic) metric presents the model’s ability to discriminate between the in-distribution and out-of-distribution data while the \textbf{AUPR} (the area under the precision-recall curve) metric measures if the model can find all out-of-distribution data without accidentally marking any in-distribution data as out-of-distribution data. \textit{For the \textbf{AUROC} and \textbf{AUPR} measures, the higher value is better}.

The source code and data samples for reproducing the experiments of our \ourapp~ method are published at \textit{\url{https://anonymous.4open.science/r/LEO/}}.

\subsection{Experimental results}\label{sec:exp_results}

\textbf{RQ1: \rqone}
\vspace{-2mm}
\paragraph{\textbf{Approach}}

We compare the performance of our \ourapp~ method with the baselines including \textbf{Standard DNN} \cite{Hendrycks2017dnn}, \textbf{Outlier Exposure} \cite{Hendrycks18}, \textbf{SSD} \cite{Sehwag21}, \textbf{VulDeePecker} \cite{VulDeePecker2018}, \textbf{CodeBERT} \cite{CodeBERT2020}, and \textbf{ReGVD} \cite{ReGVD2022} in the task of out-of-distribution vulnerability detection using FPR (at TPR 95\%), AUROC, and AUPR measures.

As mentioned, we conduct our experiments on the top five popular (CWE) vulnerability types including CWE-119 (Improper Restriction of Operations within the Bounds of a Memory Buffer), CWE-20 (Improper Input Validation), CWE-125 (Out-of-bounds Read), CWE-200 (Exposure of Sensitive Information to an Unauthorized Actor), and CWE-264 (Permissions, Privileges, and Access Controls). 


\input{tables/table1t}


In the training phase, we alternatively use each CWE vulnerability type as in-distribution data to train our \ourapp~ method and the baselines. In the inference (testing) phase, for each trained model on a specific in-distribution CWE vulnerability type, we use the remaining CWE vulnerability types as out-of-distribution data to evaluate the model's performance for out-of-distribution vulnerability detection. For example, we train each model using the CWE-119 vulnerability type as in-distribution data. In the inference (testing) phase, we use other CWE vulnerability types (CWE-20, CWE-200, CWE-125, and CWE-264) as out-of-distribution data to evaluate the model performance. We then do the same process for other CWE vulnerability types. \textbf{It is worth noting that in the training phase, we do not know and do not use any information from out-of-distribution vulnerability source code data. We only use out-of-distribution vulnerability data in the inference process for evaluating the models' performance}.

\vspace{-1mm}
\paragraph{\textbf{Quantitative results}}

The experimental results in Table 1 show the superiority of our proposed \ourapp~ method over the baseline approaches. In particular, our method obtains much higher performances in all of the used measures including FPR, AUROC, and AUPR with a high margin for almost all cases of the in-distribution data and out-of-distribution vulnerability source code data. \textit{Our \ourapp~ method is strongly effective for detecting out-of-distribution source code vulnerabilities with nearly 0\% for the FPR measure and over 90\% for both the AUROC and AUPR measures in almost all cases of the in-distribution and out-of-distribution data}. Especially, in some cases of the in-distribution and out-of-distribution data pairs, our \ourapp~ method achieves nearly 100\% for both the AUROC and AUPR measures. 

In general, to the FPR measure, our method achieves significantly higher performances than the baselines from around 1\% to 83.1\% while to the AUROC and AUPR measures, our method obtains higher performances from around (1.5\% to 16\%) and (4.9\% to 75.4\%), respectively, compared to the baseline approaches across the used in-distribution data and out-of-distribution source code vulnerabilities.

\vspace{-1mm}
\paragraph{\textbf{Qualitative results}}
To further demonstrate the advancement and effectiveness of our \ourapp~ method for OOD vulnerability detection, we visualize the representations of both in-distribution and out-of-distribution data in the feature space. This visualization helps us investigate whether our method can successfully learn the characteristics and leverage the semantic relationships inside and between source code data. It is crucial for our method to effectively distinguish between in-distribution and out-of-distribution data samples, facilitating the OOD vulnerability detection process.

We use a t-SNE \cite{tSNE2008} projection, with perplexity equal to $60$, to visualize the distributions of the in-distribution and out-of-distribution data in the feature space. \textit{As illustrated in Figure \ref{fig:t-SNE}, it becomes apparent that our \ourapp~ method significantly enhances the separation of the distributions between in-distribution and out-of-distribution data in the latent space, compared to the baselines}. These visual representations provide compelling evidence of the robustness of our \ourapp~ method in boosting the source code data representation learning facilitating the detection of out-of-distribution vulnerabilities. This also highlights our method's ability to identify hidden vulnerability patterns in both in-distribution and out-of-distribution vulnerable source code data, facilitating their differentiation in the feature space for enhancing out-of-distribution vulnerability detection.

\begin{figure*}[ht]
\begin{centering}
\includegraphics[width=0.9\textwidth]{figures/QualitativeVisualizations.pdf}
\par\end{centering}\vspace{5mm}
\caption{A 2D t-SNE projection for the data representation distribution of the in-distribution data (blue color) and the out-of-distribution vulnerable data (red color) in the latent space (i.e., where CWE20 and CWE125 are used as in-distribution data and out-of-distribution data, respectively) of our proposed \ourapp~ method and the baselines. \label{fig:t-SNE}}
\vspace{-8mm}
\end{figure*}%

\vspace{2mm}
\colorbox{gray!20}{
\begin{minipage}{0.9\columnwidth}
\textbf{In conclusion for RQ1}: The quantitative results in Table \ref{tab:my_label1t} on three main measures (i.e., FPR (at TPR 95\%), AUROC, and AUPR) and the qualitative visualizations depicted in Figure \ref{fig:t-SNE} show the effectiveness and advancement of our \ourapp~ method in achieving significantly higher performances for out-of-distribution source code vulnerability detection over the baselines. In short, our method achieves higher performances than the baselines from around (1\% to 83.1\%), (1.5\% to 16\%), and (4.9\% to 75.4\%) to the FPR (at TPR 95\%), AUROC and AUPR measures, respectively, on the used in-distribution and out-of-distribution vulnerabilities.
\end{minipage}
}
\vspace{2mm}

Please refer to the appendix, Section \ref{sec:additionale},  for the experimental results of our proposed \ourapp~ method and baselines on some other pairs of the in-distribution and out-of-distribution source code vulnerabilities in the top five popular (CWE) vulnerability types (i.e., CWE-119, CWE-20, CWE-125, CWE-200, and CWE-264).

\vspace{5mm}

\textbf{RQ2: \rqtwo}

\input{tables/table23t}

\paragraph{\textbf{Approach}}

This research question reflects different reality cases where in-distribution source code data can consist of more than one (presented in Table \ref{tab:my_label1t}) type of vulnerability. Therefore, we further investigate our proposed \ourapp~ method's performance in cases of different vulnerability types existing in the in-distribution data and observe how the model performs compared to the baselines.

For this experiment, without loss of generality, we assume that there are two and three different vulnerability types existing in the in-distribution data. When the in-distribution data has two different types of vulnerability, we conduct four cases where we assume the in-distribution data is formed by (CWE20 and CWE264), (CWE119 and CWE125), (CWE200 and CWE264), and (CWE200 and CWE125). When the in-distribution data has three different vulnerability types, we assume the in-distribution data is formed by (CWE119, CWE20, and CWE264). 

For these combinations, we simply randomly choose different CWE types (from the top five popular CWE types) to form the in-distribution data. For each case of the in-distribution data after the training process, in the inference phase, we use the remaining CWE vulnerability types as out-of-distribution data to evaluate the model's performance for out-of-distribution vulnerability detection.

\paragraph{\textbf{Results}}

The experimental results in Table \ref{tab:my_label23t} again prove the effectiveness and superiority of our \ourapp~ method compared to the baselines for out-of-distribution vulnerability detection in all various cases of the in-distribution data. Particularly, in the cases when there is more than one vulnerability type existing in the in-distribution data (e.g., two and three different vulnerability types), our  \ourapp~ method still obtains much higher performances on almost pairs of the in-distribution and out-of-distribution for the used measures. Except for the case of the in-distribution data (CWE200 and CWE264) and the out-of-distribution data (CWE125), the second highest baseline (i.e., VulDeepecker) obtains a performance close to our \ourapp~ method, in all other cases of the in-distribution and out-of-distribution data, our \ourapp~ method gains around (3.7\% to 81.8\%), (3.8\% to 15.6\%), and (5.1\% to 74.1\%) higher than the baselines on the FPR (at TPR 95\%), AUROC, and AUPR measures, respectively.

\vspace{3mm}
\colorbox{gray!20}{
\begin{minipage}{0.9\columnwidth}
\textbf{In conclusion for RQ2}: The experimental results in Table \ref{tab:my_label23t} on the FPR (at TPR 95\%), AUROC, and AUPR measures again show the superiority of our proposed \ourapp~ method over the baselines for out-of-distribution vulnerability detection on different cases regarding the various number of vulnerability types existing in the in-distribution data. In accordance with the results shown in Table \ref{tab:my_label1t}, our  \ourapp~ method still demonstrates its noticeable advancement with much higher performances compared to the baselines on the used measures in almost all cases of the in-distribution and out-of-distribution vulnerabilities.
\end{minipage}
}
\vspace{3mm}

In Figure \ref{fig:averageresults}, we present the average values of the FPR, AUROC, and AUPR measures, respectively, for our \ourapp~ method and baselines in all cases of the in-distribution and out-of-distribution vulnerabilities mentioned in Tables \ref{tab:my_label1t} and \ref{tab:my_label23t}. These average results highlight the dramatic advancement of our \ourapp~ method compared to the baselines. In short, our \ourapp~ method obtains a significantly higher performance around (49\% to 88.3\%), (18.4\% to 30.4\%), (43.2\% to 67.9\%) in the FPR, AUROC, and AUPR measures, respectively, in comparison with the baselines.

\begin{figure*}[ht]
\vspace{0mm}
\begin{centering}
\includegraphics[width=1.0\textwidth]{figures/AverageResults.pdf}
\par\end{centering}\vspace{0mm}
\caption{The average results for the FPR, AUROC, and AUPR measures, respectively, of our \ourapp~ method and baselines in all cases of the in-distribution and out-of-distribution vulnerabilities mentioned in Tables \ref{tab:my_label1t} and \ref{tab:my_label23t}. Note that for the FPR measure, the smaller value is better while for the AUROC, and AUPR measures, the higher value is better. \label{fig:averageresults}}
\vspace{-2mm}
\end{figure*}%


\vspace{2mm}
\textbf{RQ3: \rqthree}

\paragraph{\textbf{Approach}}

We compare the performance of our \ourapp~ method to itself in the cases of using and without using cluster-contrastive learning mentioned in Eq. (\ref{eq:cluster_cl}) and the data-distribution mechanism described in Eq. (\ref{eq:realx}) to investigate if these additional terms successfully boosting the source code data representation learning facilitating the out-of-distribution source code vulnerability detection. We conduct the experiment on some random pairs of the in-distribution and out-of-distribution vulnerability types as shown in Table \ref{tab:my_label2leo}. Note that in the case without using cluster-contrastive learning and data-distribution mechanism terms, we denote the method as \ourapp-w/oCD.

\vspace{-2mm}
\paragraph{\textbf{Results}}

\input{tables/table2leo}

The experimental results in Table \ref{tab:my_label2leo} show the effectiveness of cluster-contrastive learning and the data-distribution mechanism in improving the source code data representation learning process to boost the model performance for out-of-distribution source code vulnerability detection. In particular, our method with the cluster-contrastive learning and data-distribution mechanism terms (\textbf{\ourapp}) obtained considerably higher performances than itself without using these terms (denoted as \textbf{\ourapp-w/oCD}) on almost all of the used measures and the cases of the in-distribution and out-of-distribution vulnerabilities.

For the FPR measure, \ourapp~ obtains around 1.2\% to 18.7\% higher performances compared to \ourapp-w/oCD, except for the case of (CWE119 vs. CWE200) where \ourapp-w/oCD also obtains 0\% for the FPR measure. For the AUROC and AUPR measures, in all cases of the in-distribution and out-of-distribution data mentioned in Table \ref{tab:my_label2leo}, \ourapp~ achieves around (1.3\% to 7.4\%) and (3.1\% to 28.3\%) higher compared to \ourapp-w/oCD, respectively.

\vspace{3mm}
\colorbox{gray!20}{
\begin{minipage}{0.9\columnwidth}
\textbf{In conclusion for RQ3}: The experimental results mentioned in Table \ref{tab:my_label2leo} on the FPR (at TPR 95\%), AUROC, and AUPR measures show the benefits of using cluster-contrastive learning (leveraging source code characteristics and semantic vulnerability pattern relationships) and the data-distribution mechanism for boosting source code data representation learning. These terms help significantly improve the model performance for out-of-distribution vulnerability detection compared to the case without using these terms on all the used measures in almost all cases of the in-distribution and out-of-distribution vulnerabilities.

\end{minipage}
}
\vspace{3mm}

The average experimental results of the FPR, AUROC, and AUPR measures, respectively, for the \ourapp~ and  \ourapp-w/oCD methods in all cases of the in-distribution and out-of-distribution vulnerabilities mentioned in Tables \ref{tab:my_label2leo} are shown at Figure \ref{fig:averageresults_leowwt}. These values show a significant advancement of \ourapp~ over \ourapp-w/oCD in all the used metrics, especially for the FPR and AUPR measures.

\begin{figure}[ht]
\begin{centering}
\vspace{0mm}
\includegraphics[width=0.8\columnwidth]{figures/AverageResults_LEOwwt.pdf}
\par\end{centering}\vspace{1mm}
\caption{The average results for the FPR (at TPR 95\%), AUROC, and AUPR measures, respectively, of \ourapp-w/oCD and \ourapp~ in all cases of the in-distribution and out-of-distribution vulnerabilities mentioned in Table \ref{tab:my_label2leo}. \label{fig:averageresults_leowwt}}
\vspace{-2mm}
\end{figure}%

Please refer to the appendix, Section \ref{sec:discussion}, for our discussions about the threats to the validity of our proposed \ourapp~ method and corresponding mitigation.

==> usenix_version/sections/framework.tex <==
\section{The proposed \ourapp~ approach}\label{sec:framework}

\subsection{The problem statement}
We denote $D_{in}$ as a source code vulnerability type dataset consisting of $\{(X_{1}, Y_{1}),\dots,(X_{N_{D_{in}}}, Y_{N_{D_{in}}})\}$ where $X_i$ is a data sample (i.e., a function or a program) comprised of $L$ code statements from $\boldsymbol{x}_{1}$ to $\boldsymbol{x}_{L}$ while $X_i$'s vulnerability label $Y_{i}\in\{0,1\}$ (i.e., $0$: non-vulnerable and $1$: vulnerable). 
From the dataset $D_{in}$, we can build AI-based (machine learning or deep learning) approaches to detect the vulnerability (i.e., benign or vulnerable) of the source code data sampled from the distribution $D_{in}$; however, they are known to fail against the data samples (outliers or out-of-distribution) that lie far away from the training data distribution $D_{in}$ with high confidence. Advanced machine learning and deep learning approaches for OOD detection have been widely introduced, notably based on and applicable in computer vision and medical applications. These methods determine whether input data samples belong to the in-distribution or out-of-distribution category before they are input to downstream neural network modules.

The ability to identify anomalous (out-of-distribution) data plays a crucial role in ensuring the safety and dependability of predictions. In the cyber security domain, by doing this, we help the security analysts detect the new potential vulnerabilities existing in the input samples. That helps harden the software or network systems defense. \textit{In our paper, we focus on the task of detecting whether an input source code data sample is from a learned distribution $D_{in}$ or from an out-of-distribution $D_{out}$} vulnerability.

\subsection{Methodology}

In what follows,  we present the details of how our proposed \ourapp~ method works and addresses the out-of-distribution vulnerability detection problem. We first describe the process of our \ourapp~ method taking into account the source code characteristics and working to automatically learn and figure out the important and vulnerability-relevant source code statements, forming the corresponding hidden vulnerability patterns in vulnerable source code data, contributing to robust source code data representation learning for facilitating out-of-distribution source code vulnerability detection. We then present our effective solution for leveraging the semantic relationships of hidden vulnerability patterns inside and between the source code samples (i.e., functions or programs) by utilizing innovative cluster-contrastive learning to further improve the source code data representation learning process.

\begin{figure}[ht]%
\begin{centering}
\begin{tabular}{c}
\includegraphics[width=0.45\textwidth]{figures/Ourframework_v2.pdf}\tabularnewline
\end{tabular}\vspace{1mm}
\par\end{centering}
\caption{A visualization of our proposed \ourapp~ method for effectively improving the source code data representation learning process for OOD vulnerability detection.}\label{fig:deeplearning_v2}
\vspace{-5mm}
\end{figure}%

\vspace{-2mm}
\subsubsection{\textbf{Important feature selection and hidden vulnerability patterns learning}}\label{sec:selection_network}

As depicted in Figure \ref{fig:deeplearning_v2}, our \ourapp~ method starts with a selection network $\zeta$ for automatically learning and figuring out the important and vulnerability-relevant code statements in each source code data, forming the corresponding vulnerability patterns in vulnerable source code, leading to robust source code data representation learning and facilitating out-of-distribution source code vulnerability detection.

\vspace{-2mm}
\paragraph{\textbf{Motivation}}
In reality, to real-world image or text data, only some parts of the data are important and lead to the corresponding label. To illustrate, images can be modeled as backgrounds plus objects while text can be considered as a combination of high-frequency stop words plus semantic words. We witness the same property for source code data. In particular, in source code data, there are some code statements much more important than others in contributing to the vulnerability of the data, especially to vulnerable source code data samples. The core important code statements usually form the corresponding vulnerability patterns of the vulnerable source code data (i.e., \textit{please refer to Figure \ref{fig:boe_update} for examples where the core vulnerable statements are highlighted in red color}) while the vulnerability-irrelevant code statements can be shared between different vulnerable data and potentially compromise the model capability in learning the data representations of vulnerable source code samples.

\vspace{-2mm}
\paragraph{\textbf{Selection network}}

Giving a source code data sample $X$ consisting of $L$ code statements from $\mathbf{x}_{1}$ to $\mathbf{x}_{L}$ (i.e., \textit{in practice, each code statement $\mathbf{x}_{i}$ is represented as a vector using a learnable embedding method, please refer to the data processing and embedding in the appendix, Section \ref{sec:datape}, for details}), our selection network $\zeta$ aims to select the important and vulnerability label-relevant code statements $\tilde{X}$ in $X$ by learning a set of independent Bernoulli latent variables $\mathbf{z}\in\{0,1\}^{L}$. That represents the importance of the sentences to the corresponding vulnerability $Y$ of $X$. Specifically, each element $z_{i}$ in $\mathbf{z}=\{z_{i}\}_{i=1}^{L}$ indicates if $\mathbf{x}_{i}$ is related to the vulnerability $Y$ (i.e., if  $z_{i}$ is equal to $1$, the statement $\mathbf{x}_{i}$ plays an important role causing the vulnerability $Y$). Note that for the vulnerable source code data, the selected statements represent those that make the data vulnerable.

To construct $\mathbf{z}=\{z_{i}\}_{i=1}^{L}$, we model $\mathbf{z} \sim \mathrm{MultiBernoulli}(\mathbf{p}) = \prod_{i=1}^{L}\text{Bernoulli}(p_{i})$, which indicates $\mathbf{x}_{i}$ is related to the vulnerability $Y$ of $X$ with probability $p_{i}$ where $p_{i}=g_{i}\left(X;\alpha\right)$ with $g$ is a neural network parameterized by the parameter $\alpha$. It is worth noting that the neural network $g$ takes $X$ as input and outputs corresponding $\mathbf{p}=\{p_{i}\}_{i=1}^{L}$.  
With $\mathbf{z}$, we construct $\tilde{X}=\zeta\left(X\right)$ (i.e., the subset code statements that lead to the vulnerability $Y$ of the function $X$) by $\tilde{X}=X\odot \mathbf{z}$, where $\odot$ represents the element-wise product. \textit{Note that we can view the selection model as a distribution $q_{sel}(\mathbf{z}|X;\alpha)$ over a selector variable $\mathbf{z}$} which indicates the important features (i.e., code statements) for a given sample of $X$.

\begin{figure}[th]
\vspace{-1mm}
\begin{centering}
\includegraphics[scale=0.66]{figures/Selection_network_v2.pdf}
\par\end{centering}
\caption{A visualization for the selection network $\zeta$ which works as a feature selection model for robust data representation learning. Assuming that we have a source code data sample $X=[\mathbf{x}_{1},\mathbf{x}_{2},\mathbf{x}_{3},\mathbf{x}_{4},...,\mathbf{x}_{L}]$ going through the selection network (i.e., it learns a set of independent Bernoulli latent variables $\mathbf{z}\in\{0,1\}^{L}$ representing the importance of the sentences to the corresponding vulnerability $Y$ of $X$) to obtain $\mathbf{z}=[0,1,1,0,...,1]$. From $X$ and $\mathbf{z}$, we construct $\tilde{X}$ by $X\odot \mathbf{z}$. At the end, we obtain $\tilde{X}=[\mathbf{0},\mathbf{x}_{2},\mathbf{x}_{3},\mathbf{0},...,\mathbf{x}_{L}]$.}\label{fig:visualizationfor_eq_1_2}
\vspace{-2mm}
\end{figure}

\vspace{-1mm}
To make the selection process (i.e., the process consists of sampling operations from a Multi-Bernoulli distribution) continuous and differentiable during training, we apply the Gumbel-Softmax trick {\cite{jang2016categorical, MaddisonMT16}} for relaxing each Bernoulli variable $z_{i}$. Specifically, we sample $z_{i}\left(X;\alpha\right)\sim\text{Concrete}(g_{i}(X;\alpha),1-g_{i}(X;\alpha))$:

\vspace{-2mm}
\[z_{i}\left(X;\alpha\right)=\frac{\exp\{(\log g_{i}+a_{i})/\nu\}}{\exp\{(\log g_{i}+a_{i})/\nu\}+\exp\{(\log\left(1-g_{i}\right)+b_{i})/\nu\}}
\]
\vspace{-2mm}

where we denote $g_{i}\left(X;\alpha\right)$ as $g_{i}$ while $\nu$ is a temperature parameter (i.e., controlling how closely a continuous representation from a Gumbel-Softmax distribution approximates this from the corresponding discrete representation from a discrete distribution (e.g., the Bernoulli distribution)), random noises $a_{i}$ and $b_{i}$ independently drawn from \textbf{Gumbel} distribution
$G = - \log(- \log u)$ with $\ u \sim \textbf{Uniform}(0,1)$.

\vspace{-2mm}
\paragraph{\textbf{Mutual information for guiding the selection process}}
Here, we present how to use mutual information for guiding the selection network in obtaining the most meaningful $\tilde{X}$ (i.e., $\tilde{X}$ can predict the vulnerability $Y$ of $X$ correctly).

In information theory \cite{TheoryofC, EofIT2006}, mutual information is used to measure the mutual dependence between two random variables. In particular, it quantifies the information obtained about one random variable by observing the other. Leveraging this property of mutual information and inspired by \cite{learning-to-explain-l2x,van-ijcnn2021}, we maximize the mutual information between $\tilde{X}$ and $Y$ as mentioned in Eq. (\ref{eq:max_info}) with the intuition is that by using the information from $Y$, the selection process $\zeta$ will be learned and enforced to obtain the most meaningful $\tilde{X}$ (i.e., $\tilde{X}$ can predict the vulnerability $Y$ of $X$ correctly).

By viewing $\tilde{X}$ and $Y$ as random variables, \textit{the selection process (model) $\zeta$ is learned by maximizing the mutual information between $\tilde{X}$ and $Y$} as follows:

\vspace{-2mm}
{
\begin{equation}
\max_{\zeta}\,I(\tilde{X},Y).\label{eq:max_info}
\end{equation}
}
\vspace{-2mm}

Following \cite{EofIT2006}, we expand Eq. (\ref{eq:max_info}) further as the Kullback-Leibler divergence (i.e., it measures the difference in the information of two distributions) of the product of marginal distributions of $\tilde{X}$ and $Y$ from their joint distribution:

\vspace{-3mm}
{
\begin{align}
I(\tilde{X},Y)= & \int p(\tilde{X},Y)\log\frac{p(\tilde{X},Y)}{p(\tilde{X})p(Y)}d\tilde{X}dY\nonumber \\ 
\geq & \int p(Y,\tilde{X})\log\frac{q(Y|\tilde{X})}{p(Y)}dYd\tilde{X}\label{eq:1sm}
\end{align}
}
\vspace{-3mm}

In practice, estimating mutual information is challenging as we typically only have access to samples but not the underlying distributions. Therefore, in the above derivation, we apply to use a variational distribution $q(Y|\tilde{X})$ to approximate the posterior $p(Y|\tilde{X})$, hence deriving a variational lower bound of $I(\tilde{X}, Y)$ for which the equality holds if $q(Y|\tilde{X})=p(Y|\tilde{X})$. This can be further expanded as:

\vspace{-3mm}
{
\begin{align}
I(\tilde{X},Y)\geq & \int p(Y,\tilde{X},X)\log\frac{q(Y|\tilde{X})}{p(Y)}dYd\tilde{X}dX\nonumber \\
= & E_{X,Y}E_{\tilde{X}|X}[\log q(Y|\tilde{X})]+\text{const}\label{eq:2sm}
\end{align}
}
\vspace{-3mm}

To model the conditional variational distribution $q(Y|\tilde{X})$, we introduce a classifier implemented with a neural network $f(\tilde{X};\beta)$, which takes $\tilde{X}$ as input and outputs its corresponding label $Y$ (i.e., \textit{we view the classifier model as a distribution $q_{class}(Y|\tilde{X};\beta)$}). Our objective is to learn the selection process (model) as well as the classifier to maximize the following objective function:

\vspace{-3mm}
{
\begin{equation}
\underset{\alpha,\beta}{\text{max}}\left\{E_{X,Y}E_{\mathbf{z}\sim q_{sel}(\mathbf{z}|X;\alpha)}[\text{log}q_{class}(Y|X\odot\mathbf{z};\beta)]\right\}\label{eq:max_info_mutual_v2}
\end{equation}
}
\vspace{-3mm}

The mutual information facilitates a joint training process for the classifier and the selection process (model). The classifier learns to identify a subset of features leading to a data sample's label while the selection process is designed to select the best subset according to the feedback of the classifier.

\begin{figure}[th]
\vspace{0mm}
\begin{centering}
\includegraphics[scale=0.6]{figures/Mutual_information_v2.pdf}
\par\end{centering}
\vspace{1mm}
\caption{A visualization of the joint training process of the classifier and the selection model process guided by maximizing mutual information between $\tilde{X}$ and $Y$. \label{fig:visualizationfor_eq_1_2}}
\vspace{-5mm}
\end{figure}

\textit{The joint training process between the classifier $f(.,\beta)$ and the selection network $g(.,\alpha)$ brings benefits for selecting the important and label-relevant features from the corresponding data}. However, this joint training process can cause a potential limitation. 
In particular, the predictions of the classifier $f(.,\beta)$ can be based more on the features selected from the selection network $g(.,\alpha)$ than the underlying information contained in the features. In this case, the selected information (i.e., sentences) can be any subsets of the entire sentences, not the meaningful ones from the data.

\vspace{-8mm}
To solve this problem and ensure the learnable selection process respecting the data distribution in order to select both the meaningful and label-relevant information of the data, in addition to learning the classifier jointly with the selection network as mentioned in Eq. (\ref{eq:max_info_mutual_v2}), inspired by \cite{realx2021}, we propose to learn the classifier model $f(.,\beta)$ disjointly to approximate the ground truth conditional distribution of $Y$ given subsets of $X$ denoted by $X_R$ where $X_{R}=X\odot \mathbf{r}$ with $\mathbf{r}\sim \text{MultiBernoulli}(0.5)$ (denoted by $\mathbf{r}\sim \text{B}(0.5)$ for short). \textit{This procedure helps adjust the classifier to let it not just only be affected by the information obtained from the selection network but also based on the underlying information from the data to update its parameters}. We name this procedure as a \textbf{data-distribution mechanism}. This procedure is then expressed as learning $q_{class}(.;\beta)$ to maximize:

\vspace{-5mm}
{
\begin{gather}
E_{X,Y}E_{\mathbf{r}\sim \text{B}(0.5)}\{\text{log}q_{class}(Y|X\odot\mathbf{r};\beta)\}\label{eq:realx}
\end{gather}
}
\vspace{-5mm}

To make this procedure (i.e., it consists of sampling operations from a Multi-Bernoulli distribution) continuous and differentiable during training, we apply the 
Gumbel-Softmax trick {\cite{jang2016categorical, MaddisonMT16}} for relaxing each Bernoulli variable $r_{i} \in \mathbf{r}$ using RelaxedBernoulli distribution function from \cite{RelaxedBernoulli}.

\vspace{-2mm}
\subsubsection{\textbf{Innovative cluster-contrastive learning for improving source code data representation learning}}\label{sec:cluster_contrastive_learning}

\paragraph{\textbf{Motivation}}

Using contrastive learning \cite{Khosla2020} for improving data representations has been widely applied to computer vision domain applications from vision classification, detection, and segmentation \cite{NEURIPS2020_Kim, Wang_2021_ICCV, Sun_2021_CVPR, Du_2022_CVPR, Wang_2021_CVPR} to vision data out-of-distribution detection \cite{Sehwag21}. Its main idea is to encourage the data having the same label to share the close representations. \textit{We also consider if contrastive learning can help improve the source code data representation learning process.} However, via our observations, it seems to be overdoing and not appropriate when straightforwardly applying contrastive learning to the source code data because even from the same vulnerability, source code data can often consist of different hidden vulnerability patterns causing them vulnerable (in our experiment in Section \ref{sec:experiments}, we demonstrate this observation by comparing our \ourapp~ method with one of the most effective OOD approaches using contrastive learning, namely SSD \cite{Sehwag21}). 

As illustrated in Figure \ref{fig:boe_update}, although having the same vulnerability $Y$ label (e.g., vulnerability type, i.e., buffer overflow error), there are still different hidden vulnerability patterns causing the source code data samples vulnerable. Therefore, although in the same vulnerability $Y$ label, the vulnerable source code samples formed from different vulnerability patterns need to have different representations. Otherwise, when they are from the same vulnerability patterns, their representations should be close or similar. \textit{To ensure these properties and leverage the power of contrastive learning to further improve the data representation learning process,} we apply to use of innovative cluster-contrastive learning in the representation learning process of source code data.

\begin{figure}[th]
\vspace{-2mm}
\begin{centering}
\includegraphics[scale=0.43]{figures/BOE_v2.pdf}
\par\end{centering}
\vspace{3mm}
\caption{An example of different vulnerability patterns causing buffer overflow error. \textit{The left-hand figure} is an example of the buffer copy without checking the size of the input. This function allocates a buffer of 64 bytes to store the hostname; however, there is no guarantee that the hostname will not be larger than 64 bytes. If an attacker specifies an address that resolves to a very large hostname, then the function may overwrite sensitive data or even relinquish control flow to the attacker. \textit{The right-hand figure} is an example of the improper validation of an array index. This method only verifies that the given array index is less than the maximum length of the array but does not check for the minimum value. This will allow a negative value to be accepted as the input array index which will result in an out-of-bounds read and may allow access to sensitive memory. \label{fig:boe_update}}
\vspace{-5mm}
\end{figure}

\vspace{-3mm}
\paragraph{\textbf{Innovative cluster-contrastive learning.}\label{par:Clustered-spatial-contrastive}}

We notice that vulnerable source code data samples originating from the same vulnerability pattern tend to have similar $\tilde{X}$ and form the corresponding cluster in the latent space. Therefore, we use clustering analysis (e.g., $k$-means) on the representations $\tilde{X}$ of the vulnerable source code samples  in the latent space to group vulnerable  samples  with the same vulnerability patterns into clusters \textit{before employing contrastive learning to force vulnerable data to become more similar in the same clusters and to be pushed far way in different clusters} as follows:

\vspace{-2mm}
{\small{}
\begin{equation}
\mathcal{L}_{ccl} = \sum_{i\in I}1_{Y_{i}=1}\frac{-1}{\left|C(i)\right|}\sum_{c\in C(i)}\log\frac{\exp(\text{sim}({\tilde{X}_{i}},{\tilde{X}_{c}})/\tau)}{\sum\limits_{a\in A(i)}\exp(\text{sim}({\tilde{X}_{i}},{\tilde{X}_{a}})/\tau)} \label{eq:cluster_cl}
\end{equation}
}{\small\par}
\vspace{-2mm}

where $I\equiv\{1...m\}$ is a set of indices of input data in a specific mini-batch. $A(i)\equiv I\setminus\{i\}$ while $C(i)\equiv\{c\in A(i):\bar{Y}_{c}=\bar{Y}_{i}$ and $Y_{i}=1\}$ is the set of indices of vulnerable source code samples (labeled $1$) which are in the same cluster as $F_{i}$ except $i$, and $\left|C(i)\right|$ is its cardinality. Here, we apply $k$-means for each mini-batch and denote $\bar{Y}_{i}$ as the cluster label of the data sample $\tilde{X}_{i}$. For the $sim(.,.)$ function, we apply cosine similarity (please refer to the appendix, Section \ref{sec:cosines}, for details). Note that to form the corresponding vector for each $\tilde{X}_{i}$ in the latent space for calculating the cosine similarity, we simply concatenate all vectors where each vector stands for a representation of a code statement in $\tilde{X}_{i}$).


It is worth noting that cluster-contrastive learning described in Eq. (\ref{eq:cluster_cl}) helps to \textit{enforce important properties of the source code data including} (i) the vulnerable and non-vulnerable source code samples should have different representations, (ii) the vulnerable source code samples from different hidden vulnerability patterns are also encouraged to have different representations while (iii) the vulnerable source code samples in the similar hidden vulnerability patterns are trained to have close representations. Ensuring these properties definitely helps improve the selection process. That helps boost the data representation learning facilitating out-of-distribution vulnerability detection.

\subsubsection{\textbf{A summary of our proposed method}}

Please refer to Algorithm 1 for the details of our \ourapp~ method in both the training and testing phases. After the training phase, we aim to obtain the optimal selection network for the source code data representation learning. That can select the most meaningful and label-relevant features (i.e., source code statements), forming the corresponding vulnerability pattern to the vulnerable source code, for each source code data to facilitate out-of-distribution vulnerability detection.

\paragraph{The inference phase}
Inspired by \cite{Lee18b, Winkens2020, Sehwag21}, we use the cluster-conditioned out-of-distribution detection method (i.e., applying the Mahalanobis distance to calculate the outlier score $s(X)$ for each testing source code input sample $X$) in the latent space for out-of-distribution vulnerability detection. \textit{The intuition is that an effective model will produce a high-quality data representation learning process (model) for obtaining robust data representations. Therefore, in the latent space, via the data representation learning model, the representations of the in-distribution data and OOD data should be separated.}

The procedure for a cluster-conditioned detection method is as follows: We first partition the features of in-distribution training data into $K$ clusters equal to the number of clusters used in cluster-contrastive learning. We then compute the outlier score $s(X)$ of each testing input $X$ as $s(X)=min_{k}(\tilde{X}-\mu_{k})^{\mathrm{\top}}\Sigma_{k}^{-1}(\tilde{X}-\mu_{k})$ where $\mu_{k}$ and $\Sigma_{k}$ are the sample mean and sample covariance of each cluster $k$ in $K$ clusters. We finally compare this outlier score with a threshold value to decide if the corresponding input sample is out-of-distribution. 

\RestyleAlgo{ruled}
\begin{algorithm*}[htbp]
\input{sections/algorithm}\caption{The algorithm of our proposed \ourapp~ method for out-of-distribution source code vulnerability detection.\label{alg:The-training-algorithm-prom}}
\end{algorithm*}

==> usenix_version/sections/introduction.tex <==
\section{Introduction}\label{sec:introduction}

Software vulnerabilities (SVs), known as specific flaws or oversights in software programs allowing attackers to exploit the code base and potentially undertake dangerous activities (e.g., exposing sensitive information or taking control of a computer system) \cite{Dowd2006}, have become a common, serious, and crucial issue to safety-critical security. There have been many approaches proposed for software vulnerability detection (SVD) ranging from open-source to commercial tools, and from manual to automatic methods \cite{Neuhaus:2007:PVS, shin2011evaluating, yamaguchi2011vulnerability, Grieco2016, Li2016:VAV, KimWLO17, VulDeePecker2018, Duan2019, Cheng2019, nguyen2019deep, Zhuang2020, van-dual-dan-2020, van-ijcnn2021, ReGVD2022} have been proposed and implemented based on machine learning and deep learning approaches.

Although achieving significant performances for SVD and other domain applications (e.g., autonomous driving and biometric authentication), machine learning-based and deep learning-based methods are well known to fail against input data (i.e., referred to as OOD data) lying far away from the training data distribution (i.e., in-distribution). This drawback causes serious problems where the models fail to indicate when they are likely mistaken. Deep learning-based classifiers have been shown to incorrectly classify such out-of-distribution data samples into in-distribution classes with high confidence \cite{goodfellow-2014, NguyenYC14}. That can limit their adoption as well as cause unexpected crucial accidents in safety-critical systems such as medical and security domains. \textit{This problem is extremely serious in the cyber security domain. Hackers can create vulnerabilities (with the assistance of domain experts and AI-based tools, e.g., generative large language models) and exploit unknown (or out-of-distribution) vulnerabilities to compromise computer or network systems until appropriate measures are taken to address and mitigate the issue}.

The problems of out-of-distribution (also known as anomaly or outlier) result in rapid progress in the use of advanced machine learning and deep learning for out-of-distribution (OOD) detection before feeding input data samples to the downstream AI-based modules. However, though achieving significantly promising performance for OOD detection, almost all existing methods are mainly based on or applicable to images in computer vision (e.g., \cite{HendrycksG16c, Hendrycks18, Lee18a, Lee18b, Sehwag21, sun2022outofdistribution}) or genomics sequences in medical diagnosis (e.g., \cite{Ren19}), automated deep learning-based techniques for OOD source code vulnerability detection have not yet been well studied and explored. Furthermore, we observed that these methods cannot be straightforwardly applied in the context of out-of-distribution source code vulnerability detection due to the difference in the nature of source code data compared with images and genomics sequences. Motivated by this problem, in this paper, we study the research questions:

\vspace{1mm}
\colorbox{gray!10}{
\begin{minipage}{0.9\columnwidth}
"How to derive an effective method for out-of-distribution (OOD) source code vulnerability detection where we aim to detect if an input source code data is from an out-of-distribution vulnerability? What are the main challenges and key characteristics of source code data to be considered?"
\end{minipage}
}
\vspace{1mm}

We notice that various instances of vulnerable source code data, associated with different vulnerability types (e.g., buffer overflow error or resource management error), frequently originate from distinct vulnerability patterns. In each source code data sample (i.e., a function or a program), the vulnerability pattern emerges from the intricate semantic relationships between vulnerability-relevant source code statements. \textit{Therefore, to be able to figure out the difference between source code data from various vulnerabilities to facilitate OOD vulnerability detection, the corresponding method definitely should have the capability of learning and figuring out the important source code statements that form the vulnerability patterns of the associated vulnerable source code data.}

When it comes to source code data, we observed some key characteristics as follows: (i) source code data (i.e., functions or programs) are complicated and different from texts or images due to consisting of complex semantic and syntactic relationships between code statements and code tokens forming the corresponding vulnerability, (ii) different source code data can share a lot of common background information (e.g., non-vulnerable code sentences) while there are only a few sentences causing the data to be different and vulnerable. This problem requires an appropriate solution to learn and figure out vulnerable parts inside vulnerable data for being able to distinguish non-vulnerable and vulnerable source code data samples, and (iii) although having the same vulnerability label (e.g., vulnerability type, i.e., buffer overflow error, or vulnerable one in general), there are still many different hidden vulnerability patterns causing the source code data samples vulnerable. Therefore, an elegant mechanism for automatically figuring out and separating the vulnerable source code samples consisting of different vulnerability patterns is also needed to have robust data representation learning for OOD source code vulnerability detection.

To this end, in this paper, we propose a novel deep learning-based approach that can learn and leverage the characteristics of source code data to automatically figure out the important and vulnerability-relevant code statements, forming the corresponding hidden vulnerability patterns of vulnerable source code data. In addition, our approach can also utilize the semantic relationships of hidden vulnerability patterns inside and between source code data samples to boost the data representation learning for OOD source code vulnerability detection. Via this paper, we demonstrate that \textit{the ability to capture the characteristics of source code data as well as figure out and leverage the relationships of hidden vulnerability patterns inside and between source code data samples for boosting the data representation learning play a key role for OOD source code vulnerability detection}.

In particular, our approach consists of two phases. \textbf{In the training phase}, we propose an elegant training principle based on information theory and cluster-contrastive learning for effectively learning and leveraging the characteristics of source code data to boost the data representation learning process.
During the training phase, our proposed approach enhances the learning of semantic relationships inside and between source code data samples for forming clear boundaries between source code data consisting of different hidden vulnerability patterns (i.e., \textit{note that in the latent space, the representations of vulnerable source code data sharing the same hidden vulnerability pattern tend to form a corresponding cluster}) in the latent space for the training set of the in-distribution data ($D_{in}$). \textbf{In the testing (inference) phase}, inspired by \cite{Lee18b, Winkens2020, Sehwag21}, 
we use the cluster-conditioned detection method (using the Mahalanobis distance \cite{Mahalanobis}) to calculate the outlier score $s(X)$ for each testing input data sample $X$ in the latent space with respect to the training data set (i.e., $D_{in}$). Based on the outlier score $s(X)$, we determine whether $X$ is out-of-distribution. Please refer to Section \ref{sec:framework} for a comprehensive explanation, visualization, and algorithm of our proposed method.

\vspace{1mm}
In summary, our key contributions are as follows:
\begin{itemize}
\item We study an important problem of out-of-distribution source code vulnerability detection. Automated machine learning and deep learning-based techniques for this problem have not yet been well studied and explored.
\item We propose an innovative end-to-end deep learning-based framework derived from an information-theoretic perspective integrated with innovative cluster-contrastive learning for automatically learning the characteristics of source code data. Our framework can also figure out and leverage the semantic relationships of hidden vulnerability patterns inside and between source code data (e.g., functions or programs) to boost the data representation learning for OOD source code vulnerability detection. \textit{To the best of our knowledge, our work is one of the first methods proposed to solve the problem.}
\item We comprehensively evaluate and compare our proposed approach with different state-of-the-art baselines on real-world source code datasets. Our extensive experiments show that our proposed approach obtains a significantly higher performance than the baselines in three main measures including FPR (at TPR 95\%), AUROC, and AUPR, used in almost all of the out-of-distribution detection methods, notably \cite{Hendrycks18, Ren19, Sehwag21}.

\end{itemize}

==> usenix_version/sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}
\paragraph{\textbf{OOD detection}}

There have been many AI-based methods (i.e., machine learning-based and deep learning-based approaches) introduced for out-of-distribution detection widely applied to computer vision and medical diagnosis applications. While traditional methods, e.g., one-class SVMs \cite{Scholkopf1999}, have been revisited with deep representations \cite{pmlr-v80-ruff18a}, yielding improvements to complex data, the vast majority of deep learning existing efforts toward developing efficient detection solutions have studied threshold-based detectors \cite{HendrycksG16c, LiangLS17, GuoPSW17, Lakshminarayanan-2016} using the confidence (or entropy) of the predictive distribution $p(Y|X)$ (where $Y$ denotes the label of the corresponding data $X$) of (or assembles of) discriminative classifiers trained on in-distribution data. Lee et al.\cite{Lee18a} and Hendrycks et al. \cite{Hendrycks18} further introduced confidence losses that use an auxiliary dataset (i.e., a generative adversarial network (GAN) \cite{goodfellow-2014} for generating the most effective samples from $P_{out}$ (out-of-distribution) or a dataset entirely disjoint from test-time data) to teach the network better representations for anomaly detection. Lee et al. \cite{Lee18b} proposed a method that is applicable to any pre-trained softmax neural classifier (without re-training) for detecting abnormal test samples including OOD and adversarial ones. In particular, the idea is to measure the probability density of the test sample on feature spaces of DNNs utilizing the concept of a generative (distance-based) classifier. 

Recently, Hendrycks et al. \cite{Hendrycks2019} proposed a method using self-supervised learning with image rotation prediction for enabling the detection of out-of-distribution examples while Winkens et al. \cite{Winkens2020} introduced a contrastive training (in addition to supervised classification losses) on image data for out-of-distribution detection. Sehwag et al. \cite{Sehwag21} proposed an outlier detector using self-supervised representation learning \cite{TingChen-2020, YonglongTian-2020} followed by a Mahalanobis distance-based detection in the feature space.

An alternative for out-of-distribution detection is to use generative model-based methods, which are appealing as they do not require labeled data and can directly model the input data distribution. Specifically, these methods fit a generative model 
to the input data and then evaluate the likelihood of new inputs under that model. However, some later works (e.g., \cite{Nalisnick18} and \cite{Choi18}) have highlighted significant issues with this approach for OOD detection on images, showing that deep generative models such as Glow \cite{Kingma18} and PixelCNN \cite{OordKK16, SalimansKCK17} sometimes assign higher likelihoods to OOD than in-distribution inputs. Ren et al. \cite{Ren19} proposed a likelihood ratio method that uses a background model to correct the background statistics and enhances the in-distribution specific features for OOD detection applied to images and genomics sequences data.

Although most of the existing methods have achieved promising results for out-of-distribution detection,  they are mainly based on or only applicable to computer vision applications or medical diagnosis. Automated deep learning-based techniques for out-of-distribution source code vulnerability detection have not yet been well studied. \textit{In our paper, we adapt some state-of-the-art out-of-distribution detection methods (e.g., \cite{Hendrycks2017dnn, Hendrycks18, Sehwag21}) to the out-of-distribution source code vulnerability detection and compare these model's performance to our proposed method}. Please refer to the Experiment section (Section \ref{sec:experiments}) for details.

\vspace{-2mm}
\paragraph{\textbf{Software vulnerability detection}}

AI-based approaches have been proposed for software vulnerability detection (SVD). Most previous work in SVD, such as \cite{yamaguchi2011vulnerability, shin2011evaluating, Li2016:VAV, Grieco2016, KimWLO17}, was based primarily on handcrafted features manually chosen by knowledgeable domain experts with possibly outdated experience and underlying biases. In many situations, these handcrafted features do not generalize well. For example, features that work well in a certain software project may not perform well in other projects \cite{Zimmermann2009}. To alleviate the dependency on handcrafted features, the use of automatic features in SVD has been studied recently \cite{VulDeePecker2018,jun_2018, Dam2018, Li2018SySeVR, Duan2019, Cheng2019, Zhuang2020, ReGVD2022}. These methods show the advantages of employing automatic features over handcrafted features for SVD. 

Although achieving significant performances in many domain applications (e.g., autonomous driving, biometric authentication, and cyber security), AI-based methods are well-known to fail against the input data lying far away from the training data distributions. In our paper, we want to investigate if effective work in SVD can produce a good performance on out-of-distribution source code vulnerability detection.

Additional baselines of our proposed method are some effective and state-of-the-art methods for software vulnerability detection including \cite{VulDeePecker2018, ReGVD2022, CodeBERT2020}. As mentioned, we aim to investigate how these methods perform for out-of-distribution source code vulnerability detection. \textbf{VulDeePecker} \cite{VulDeePecker2018} is considered one of the most effective deep learning-based software vulnerability detection methods leveraging the power of bi-directional long-short-term memory (LSTM) networks. \textbf{CodeBERT} \cite{CodeBERT2020} is a pre-trained model (based on the Transformer's encoder framework \cite{transformers-Vaswani17}) that specializes in the programming language. Via CodeBERT, we aim to investigate how large language models work in the context of out-of-distribution vulnerability detection. \textbf{ReGVD} \cite{ReGVD2022} is a simple yet effective graph neural network-based model for the software vulnerability detection problem.

==> usenix_version/tables/table1t.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.93\columnwidth}{!}{
%{|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 
%\hline 

\multirow{7}{*}{CWE20 vs. CWE119}
 &  Standard DNN & 86.15\%	& 82.78\% & 58.66\% 
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  83.49\%	& 84.02\% & 61.16\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 87.50\%	& \underline{86.89\%} & 63.45\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{34.95\%}	& 85.23\% & \underline{82.07\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT &  89.08\% & 46.34\% & 37.46\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD &  93.35\%	& 59.07\% & 39.78\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.89\%} & \textbf{99.28\%}
 %\tabularnewline

   & \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.89\%} & \textbf{99.28\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 34.95\%)} & \textcolor{blue}{($\uparrow$ 13\%)} & \textcolor{blue}{($\uparrow$ 17.21\%)}\tabularnewline
 
\hline 
%\hline 

 \multirow{7}{*}{CWE20 vs. CWE125}
 &  Standard DNN & 82.62\%	& 84.88\%	& 30.01\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  81.25\%	& 85.39\%	& 31.87\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 85.35\%	& 88.33\%	& 34.83\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{77.34\%}	& \underline{92.16\%}	& \underline{43.42\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 86.23\%	& 46.55\%	& 17.67\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 78.39\%	& 78.49\%	& 28.27\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 
 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.94\%} & \textbf{98.84\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.93\%} & \textbf{98.81\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 77.34\%)} & \textcolor{blue}{($\uparrow$ 7.77\%)} & \textcolor{blue}{($\uparrow$ 55.39\%)}\tabularnewline
 
 \hline
 %\hline
 
\multirow{7}{*}{CWE264 vs. CWE200}
 &  Standard DNN & 85.16\%	&  75.76\%	&  29.20\% 
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  79.95\%	&  85.93\%	&  39.58\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 87.76\%	&  85.22\%	&  34.04\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{1.04\%}	&  \underline{98.39\%}	&  85.52\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT  &  9.94\%	& 95.89\%	&  \underline{93.42\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  &  84.47\%	&  77.32\%	&  33.64\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 

 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.84\%} & \textbf{98.33\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.84\%} & \textbf{98.33\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 1.04\%)} & \textcolor{blue}{($\uparrow$ 1.45\%)} & \textcolor{blue}{($\uparrow$ 4.91\%)}\tabularnewline
 
 \hline
 %\hline 

 \multirow{7}{*}{CWE119 vs. CWE264}
 &  Standard DNN & \underline{83.07\%}	& 77.69\%	& 16.54\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  87.50\%	& 77.98\%	& 15.21\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 85.68\%	& \underline{84.24\%}	& \underline{20.56\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & 95.83\%	& 63.35\%	& 9.39\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 91.75\%	& 74.06\%	& 15.51\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 88.66\%	& 66.60\%	& 14.11\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
% & \ourapp~ (Ours)  &  \textbf{0.00\%}	& \textbf{99.85\%} & \textbf{95.64\%}
% \tabularnewline

  & \multirow{2}{*}{LEO (Ours)} &  \textbf{0.00\%}	& \textbf{98.62\%} & \textbf{75.18\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 83.07\%)} & \textcolor{blue}{($\uparrow$ 14.38\%)} & \textcolor{blue}{($\uparrow$ 54.62\%)}\tabularnewline
 
\hline 

\multirow{7}{*}{CWE119 vs. CWE125}
&  Standard DNN & 89.06\%	& 82.08\%	& 21.41\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure &  84.18\%	& 83.40\% & 23.37\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 87.50\%	& \underline{83.94\%}	& \underline{23.73\%}
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 96.09\%	& 67.96\%	& 13.23\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 93.12\%	& 74.18\%	& 18.47\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD & \underline{76.29\%}	& 73.37\%	& 23.46\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  \multirow{2}{*}{\ourapp~ (Ours)}  & \textbf{0.00\%} & \textbf{99.96\%} & \textbf{99.12\%}
\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 76.29\%)} & \textcolor{blue}{($\uparrow$ 16.02\%)} & \textcolor{blue}{($\uparrow$ 75.39\%)}\tabularnewline
\hline

\multirow{7}{*}{CWE200 vs. CWE20}
 &  Standard DNN & 93.16\%	& 69.00\%	& 48.74\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  88.96\%	& 77.53\%	& 56.97\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  SSD & 88.77\%	& 79.21\%	& 59.17\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  VulDeePecker & \underline{39.06\%}	& \underline{89.05\%}	& \underline{86.40\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 43.73\%	& 80.58\%	& 81.04\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD & 90.21\%	& 73.46\%	& 57.68\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.33\%} & \textbf{98.08\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.33\%} & \textbf{98.08\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 39.06\%)} & \textcolor{blue}{($\uparrow$ 10.28\%)} & \textcolor{blue}{($\uparrow$ 11.68\%)}\tabularnewline
 
 \hline
%\hline
 
\hline
\end{tabular}}
\vspace{-2mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each out-of-distribution (OOD) vulnerability corresponding with specific in-distribution (ID) data.  (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method over the second-best values from the baselines.)}\label{tab:my_label1t}
\vspace{-2mm}
\end{table}



==> usenix_version/tables/table23t.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.93\columnwidth}{!}{
% {|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 

\multirow{7}{*}
 &  Standard DNN & 92.97\%	& 75.84\%	& 37.33\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  87.55\%	& 82.12\%	& 45.63\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE20-264}
 &  SSD & 90.89\%	& 84.99\%	& 47.47\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE119}
 &  VulDeePecker & \underline{3.70\%}	& \underline{96.01\%}	& \underline{84.14\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 93.30\%	& 54.48\%	& 28.38\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 68.50\%	& 86.58\%	& 42.45\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
%&  \ourapp~ (Ours)  &  \textbf{0.00\%}	& \textbf{99.76\%} & \textbf{98.28\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO (Ours)} &  \textbf{0.00\%}	& \textbf{99.76\%} & \textbf{98.28\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 3.70\%)} & \textcolor{blue}{($\uparrow$ 3.75\%)} & \textcolor{blue}{($\uparrow$ 14.14\%)}\tabularnewline
 
\hline 
%\hline 
   
\multirow{7}{*}
 &  Standard DNN & 93.26\%	& 64.11\% & 17.91\% 
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  91.02\%	& 73.75\% & 22.57\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE119-125}
 &  SSD & 62.40\% & 61.79\% & 47.13\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE20}
 &  VulDeePecker & \underline{30.76\%}	& \underline{84.38\%} & \underline{49.47\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT &  91.22\% & 51.69\% & 19.92\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD &  90.30\%	& 70.07\% & 21.02\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.35\%} & \textbf{90.29\%}
 %\tabularnewline

& \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.97\%} & \textbf{99.66\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 30.76\%)} & \textcolor{blue}{($\uparrow$ 15.59\%)} & \textcolor{blue}{($\uparrow$ 50.19\%)}\tabularnewline
\hline 
%\hline 
  
 \multirow{7}{*}
 &  Standard DNN & 89.84\%	& 78.55\%	& 23.44\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  83.59\%	& 86.94\%	& 31.12\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE200-264}
 &  SSD & 52.34\%	& 72.17\%	& 56.15\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{vs. CWE125}
 &  VulDeePecker & \underline{0.2\%}	& \underline{99.78\%}	& \underline{98.86\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 4.97\%	& 97.52\%	& 96.02\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 75.00\%	& 83.86\%	& 31.86\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.93\%} & \textbf{99.03\%}
 %\tabularnewline
 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.93\%} & \textbf{99.03\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 0.2\%)} & \textcolor{blue}{($\uparrow$ 0.15\%)} & \textcolor{blue}{($\uparrow$ 0.17\%)}\tabularnewline
 \hline
 %\hline

  \multirow{7}{*}
 &  Standard DNN & 92.71\%	& 66.35\%	& 16.05\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  92.71\%	& 76.14\%	& 19.77\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE200-125}
 &  SSD & 88.54\%	& 74.30\%	& 20.41\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
vs. {CWE264}
 &  VulDeePecker & 79.43\%	& 67.67\%	& 22.01\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & \underline{17.53\%}	& \underline{92.91\%}	& \underline{87.71\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 90.53\%	& 60.49\%	& 18.21\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.26\%} & \textbf{99.75\%} & \textbf{92.44\%}
 %\tabularnewline
 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.78\%} & \textbf{99.47\%} & \textbf{92.85\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 16.75\%)} & \textcolor{blue}{($\uparrow$ 6.56\%)} & \textcolor{blue}{($\uparrow$ 5.14\%)}\tabularnewline
 \hline
 
 \multirow{7}{*}
 &  Standard DNN & \underline{82.03\%}	& \underline{88.01\%}	& 12.33\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  83.85\%	& 82.56\%	& 9.25\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE119-20-264}
 &  SSD & 86.46\%	& 77.02\%	& 7.37\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
vs. {CWE200}
 &  VulDeePecker & 90.10\%	& 42.56\%	& 3.03\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 90.48\%	& 48.26\%	& \underline{18.37\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 89.26\%	& 69.80\%	& 7.92\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.26\%} & \textbf{99.75\%} & \textbf{92.44\%}
 %\tabularnewline
 & \multirow{2}{*}{LEO (Ours)} & \textbf{0.26\%} & \textbf{99.75\%} & \textbf{92.44\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 81.77\%)} & \textcolor{blue}{($\uparrow$ 11.74\%)} & \textcolor{blue}{($\uparrow$ 74.07\%)}\tabularnewline
 \hline
\end{tabular}}
\vspace{-2mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each out-of-distribution (OOD) vulnerability corresponding with specific in-distribution (ID) data. (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method over the second-best values from the baselines.)}\label{tab:my_label23t}
\vspace{-2mm}
\end{table}


==> usenix_version/tables/table2app.tex <==
\begin{table}[ht]
\centering{}
\resizebox{0.93\columnwidth}{!}{
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD Datasets} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$& \textbf{AUROC} $\uparrow$& \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 
 
\multirow{7}{*}{CWE20 vs. CWE264}
&  Standard DNN & 89.58\%	& 76.48\%	& 17.40\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure & 91.93\% &  78.86\% &  18.00\%  
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 88.28\%	& 86.27\%	& 26.44\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & \underline{72.14\%}	& \underline{92.33\%}	& \underline{37.41\%}
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 90.31\%	& 48.86\%	& 13.21\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD & 91.13\%	& 63.96\%	& 15.80\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  \multirow{2}{*}{\ourapp~ (Ours)}  & \textbf{0.00\%} & \textbf{99.63\%} & \textbf{92.77\%}
\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 72.14\%)} & \textcolor{blue}{($\uparrow$ 7.3\%)} & \textcolor{blue}{($\uparrow$ 55.36\%)}\tabularnewline
\hline

\multirow{7}{*}{CWE200 vs. CWE119}
&  Standard DNN & 88.02\%	& 77.84\%	& 71.74\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure &  84.79\%	& 82.74\%	& 76.94\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 88.23\%	& 80.88\%	& 74.28\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & \underline{24.58\%}	& \underline{94.60\%}	& \underline{95.49\%}
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & 58.16\%	& 72.91\% & 80.98\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 95.58\%	& 55.13\%	& 56.73\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
%&  \ourapp~ (Ours)  & \textbf{0.00\%} & \textbf{99.32\%} & \textbf{99.05\%}
%\tabularnewline

& \multirow{2}{*}{LEO (Ours)} & \textbf{0.00\%} & \textbf{99.32\%} & \textbf{99.05\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 24.58\%)} & \textcolor{blue}{($\uparrow$ 4.72\%)} & \textcolor{blue}{($\uparrow$ 3.56\%)}\tabularnewline

 \hline
\multirow{7}{*}{CWE200 vs. CWE264}
&  Standard DNN & 93.49\%	& 67.11\%	& 25.40\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure &  91.67\%	& 75.52\%	& 31.59\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 87.24\%	& \underline{80.50\%}	& 37.54\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 65.36\%	& 74.24\%	& 53.21\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & \underline{60.00\%}	& 70.74\%	& \underline{57.74\%}
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 95.46\%	& 54.03\%	& 23.88\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  \multirow{2}{*}{\ourapp~ (Ours)}  & \textbf{0.00\%} & \textbf{99.91\%} & \textbf{99.26\%}
\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 60.00\%)} & \textcolor{blue}{($\uparrow$ 19.41\%)} & \textcolor{blue}{($\uparrow$ 41.52\%)}\tabularnewline
\hline

%\hline
\multirow{7}{*}{CWE264 vs. CWE20}
&  Standard DNN & 91.80\%	& 62.03\%	& 38.20\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  Outlier Exposure &  83.50\% &  72.09\% & 48.95\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  SSD & 85.84\%	& 82.97\%	& 59.62\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  VulDeePecker & 52.34\%	& 90.88\%	& 74.79\%
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  CodeBERT  & \underline{10.06\%}	& \underline{95.57\%}	& \underline{95.31\%}
\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  ReGVD  & 90.12\%	& 68.36\%	& 43.88\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
&  \multirow{2}{*}{\ourapp~ (Ours)}  & \textbf{0.00\%} & \textbf{99.82\%} & \textbf{99.32\%}
\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 10.06\%)} & \textcolor{blue}{($\uparrow$ 4.25\%)} & \textcolor{blue}{($\uparrow$ 4.01\%)}\tabularnewline
\hline
%\hline

 \multirow{7}{*}
 &  Standard DNN & 80.08\%	& \underline{90.47\%}	& 18.27\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  Outlier Exposure &  86.52\%	& 85.44\%	& 12.84\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
{CWE119-20-264}
 &  SSD & 94.34\%	& 79.86\%	& 9.32\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
vs. {CWE125}
 &  VulDeePecker & \underline{54.69\%}	& 88.76\%	& \underline{33.41\%}
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  CodeBERT & 90.06\%	& 47.02\%	& 19.17\%
 \tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 &  ReGVD  & 87.02\%	& 69.85\%	& 8.35\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 %&  \ourapp~ (Ours)  & \textbf{0.26\%} & \textbf{99.75\%} & \textbf{92.44\%}
 %\tabularnewline
 & \multirow{2}{*}{\ourapp~ (Ours)} & \textbf{0.00\%} & \textbf{99.93\%} & \textbf{97.06\%}\tabularnewline
%\cline{3-5} \cline{4-5} \cline{5-5} 
 &  & \textcolor{blue}{($\downarrow$ 54.69\%)} & \textcolor{blue}{($\uparrow$ 9.46\%)} & \textcolor{blue}{($\uparrow$ 63.65\%)}\tabularnewline
 \hline
\end{tabular}}
\vspace{-1mm}
\caption{The results of our \ourapp~ method and baselines for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code samples of each out-of-distribution data with the corresponding used in-distribution data. (The best results are in \textbf{bold} while the second highest results are in \underline{underline}. The numbers highlighted in blue color are the improvements of our method \ourapp~ over the second-best values from the baselines.)}\label{tab:my_label_app}
\vspace{-3mm}
\end{table}

==> usenix_version/tables/table2leo.tex <==
\begin{table}[ht]
\centering{}
\vspace{0mm}
\resizebox{0.95\columnwidth}{!}{
% {|c|c|r|r|r|}
\begin{tabular}{ccrrr}
\hline 
%\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\textbf{ID and OOD} & \textbf{Methods} & \textbf{FPR} $\downarrow$ & \textbf{AUROC} $\uparrow$ & \textbf{AUPR} $\uparrow$
\tabularnewline
\hline 

\multirow{2}{*}
 &  \ourapp-woCD & 0.00\%	& 98.55\%	& 75.44\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} {CWE119 vs. CWE200}
 %&  \ourapp  &  \textbf{0.00\%}	& \textbf{99.85\%} & \textbf{95.64\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO}  &  0.00\%	& \textbf{99.85\%} & \textbf{95.64\%}\tabularnewline
 &  & & \textcolor{blue}{($\uparrow$ 1.3\%)} & \textcolor{blue}{($\uparrow$ 20.2\%)}\tabularnewline
 
\hline 
%\hline 
 
\multirow{2}{*}
 &  \ourapp-w/oCD &  18.70\%	& 92.45\% & 84.79\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} {CWE20 vs. CWE119}
 %&  \ourapp  & \textbf{0.00\%} & \textbf{99.89\%} & \textbf{99.28\%}
 %\tabularnewline

  & \multirow{2}{*}{LEO}  & \textbf{0.00\%} & \textbf{99.89\%} & \textbf{99.28\%}\tabularnewline 
 &  & \textcolor{blue}{($\downarrow$ 18.70\%)} & \textcolor{blue}{($\uparrow$ 7.44\%)} & \textcolor{blue}{($\uparrow$ 14.49\%)}\tabularnewline
\hline 
%\hline 

\multirow{2}{*}
& \ourapp-w/oCD & 3.32\%	& 97.48\%	& 86.70\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} {CWE20 vs. CWE125}
%&  \ourapp  & 0.00\% & \textbf{99.94\%} & \textbf{98.84\%}
%\tabularnewline

 & \multirow{2}{*}{LEO}  & \textbf{0.00\%} & \textbf{99.93\%} & \textbf{98.81\%}\tabularnewline
 & & \textcolor{blue}{($\downarrow$ 3.32\%)} & \textcolor{blue}{($\uparrow$ 2.45\%)} & \textcolor{blue}{($\uparrow$ 12.11\%)}\tabularnewline
\hline
%\hline
 
\multirow{2}{*}
 &  \ourapp-w/oCD &  17.45\%	&  94.80\%	&  83.00\%
 \tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} {CWE264 vs. CWE200}
 %&  \ourapp  & 0.00\% & \textbf{99.84\%} & \textbf{98.33\%}
 %\tabularnewline

 & \multirow{2}{*}{LEO}  & \textbf{0.00\%} & \textbf{99.84\%} & \textbf{98.33\%}\tabularnewline
 & & \textcolor{blue}{($\downarrow$ 17.45\%)} & \textcolor{blue}{($\uparrow$ 5.04\%)} & \textcolor{blue}{($\uparrow$ 15.33\%)}\tabularnewline
 \hline
 %\hline 

\multirow{2}{*}
&  \ourapp-w/oCD & 1.15\% & 97.67\%	& 95.93\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} {CWE200 vs. CWE119}
%&  \ourapp  & 0.00\% & \textbf{99.33\%} & \textbf{98.08\%}
%\tabularnewline

& \multirow{2}{*}{LEO}  & \textbf{0.00\%} & \textbf{99.39\%} & \textbf{99.05\%}\tabularnewline
 & & \textcolor{blue}{($\downarrow$ 1.15\%)} & \textcolor{blue}{($\uparrow$ 1.72\%)} & \textcolor{blue}{($\uparrow$ 3.12\%)}\tabularnewline
\hline

\multirow{2}{*}{CWE200-125}
&  \ourapp-w/oCD & 9.38\% & 96.78\%	& 64.54\%
\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}
%&  \ourapp  & 0.00\% & \textbf{99.33\%} & \textbf{98.08\%}
%\tabularnewline

& \multirow{2}{*}{LEO}  & \textbf{0.78\%} & \textbf{99.47\%} & \textbf{92.85\%}\tabularnewline {vs. CWE264}
 & & \textcolor{blue}{($\downarrow$ 8.6\%)} & \textcolor{blue}{($\uparrow$ 2.69\%)} & \textcolor{blue}{($\uparrow$ 28.31\%)}\tabularnewline
\hline

%\multirow{2}{*}{CWE200 vs CWE119}
%&  Ours (w/o) & 0.05\% & \textbf{99.55\%}	& 99.02\%
%\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
%&  Ours  & \textbf{0.00\%} & 99.32\% & \textbf{99.05\%}
%\tabularnewline
%\hline
\end{tabular}}
\vspace{-1mm}
\caption{The results of our method for the FPR (at TPR 95\%), AUROC, and AUPR measures on the vulnerable source code of each OOD vulnerability corresponding with specific in-distribution (ID) data when using and without using the cluster-contrastive learning and the data-distribution mechanism. (The higher results for each measure in each pair of the ID and OOD data are in \textbf{bold}. The numbers highlighted in the blue color are the improvements of \ourapp~ over \ourapp-w/oCD.)}\label{tab:my_label2leo}
\vspace{-2mm}
\end{table}
